A projected super-penalty method for the $C^1$-coupling of multi-patch isogeometric Kirchhoff plates

This work focuses on the development of a super-penalty strategy based on the $L^2$-projection of suitable coupling terms to achieve $C^1$-continuity between non-conforming multi-patch isogeometric Kirchhoff plates. In particular, the choice of penalty parameters is driven by the underlying perturbed saddle point problem from which the Lagrange multipliers are eliminated and is performed to guarantee the optimal accuracy of the method. Moreover, by construction, the method does not suffer from locking also on very coarse meshes. We demonstrate the applicability of the proposed coupling algorithm to Kirchhoff plates by studying several benchmark examples discretized by non-conforming meshes. In all cases, we recover the optimal rates of convergence achievable by B-splines where we achieve a substantial gain in accuracy per degree-of-freedom compared to other choices of the penalty parameters.

==> pictures/numericalExamples/graphs/convergence_bilaplace_3patches_conforming_h1.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=5.75cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^1$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west,
%skip coords between index={7}{8}
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/bilaplace_penalty_curved_3patch_non_conforming_matching_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/bilaplace_penalty_curved_3patch_non_conforming_matching_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

%	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_non_matching_no_proj_breitenberger_SIMPLE_ILU_p4.txt};
%    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/bilaplace_penalty_curved_3patch_non_conforming_matching_josef_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/bilaplace_penalty_curved_3patch_non_conforming_matching_josef_p3.txt};
    \addlegendentry{$p=3$ scaled};

%	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_non_matching_no_proj_SIMPLE_ILU_p4.txt};
%    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/bilaplace_penalty_curved_3patch_non_conforming_matching_proj_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/bilaplace_penalty_curved_3patch_non_conforming_matching_proj_p3.txt};
    \addlegendentry{$p=3$ proj};

%	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_non_matching_proj_SIMPLE_ILU_p4.txt};
%    \addlegendentry{$p=4$ proj};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.365}{2}{black};
\logLogSlopeReverseTriangle{0.81}{0.08}{0.065}{3}{black};
%\logLogSlopeReverseTriangle{0.54}{0.08}{0.065}{3}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_bilaplace_3patches_conforming_h2.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=5.75cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^2$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west,
%skip coords between index={7}{8}
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_curved_3patch_non_conforming_matching_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_curved_3patch_non_conforming_matching_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

%	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_non_matching_no_proj_breitenberger_SIMPLE_ILU_p4.txt};
%    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_curved_3patch_non_conforming_matching_josef_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_curved_3patch_non_conforming_matching_josef_p3.txt};
    \addlegendentry{$p=3$ scaled};

%	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_non_matching_no_proj_SIMPLE_ILU_p4.txt};
%    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_curved_3patch_non_conforming_matching_proj_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_curved_3patch_non_conforming_matching_proj_p3.txt};
    \addlegendentry{$p=3$ proj};

%	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_non_matching_proj_SIMPLE_ILU_p4.txt};
%    \addlegendentry{$p=4$ proj};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.51}{1}{black};
\logLogSlopeReverseTriangle{0.82}{0.08}{0.065}{2}{black};
%\logLogSlopeReverseTriangle{0.54}{0.08}{0.065}{3}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_bilaplace_3patches_conforming_l2.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=5.75cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $L^2$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west,
%skip coords between index={7}{8}
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/bilaplace_penalty_curved_3patch_non_conforming_matching_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/bilaplace_penalty_curved_3patch_non_conforming_matching_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

%	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_non_matching_no_proj_breitenberger_SIMPLE_ILU_p4.txt};
%    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/bilaplace_penalty_curved_3patch_non_conforming_matching_josef_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/bilaplace_penalty_curved_3patch_non_conforming_matching_josef_p3.txt};
    \addlegendentry{$p=3$ scaled};

%	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_non_matching_no_proj_SIMPLE_ILU_p4.txt};
%    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/bilaplace_penalty_curved_3patch_non_conforming_matching_proj_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/bilaplace_penalty_curved_3patch_non_conforming_matching_proj_p3.txt};
    \addlegendentry{$p=3$ proj};

%	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_non_matching_proj_SIMPLE_ILU_p4.txt};
%    \addlegendentry{$p=4$ proj};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.365}{2}{black};
\logLogSlopeReverseTriangle{0.81}{0.08}{0.065}{4}{black};
%\logLogSlopeReverseTriangle{0.54}{0.08}{0.065}{3}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_bilaplace_9patches_conforming_h1.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.775\textwidth,
height=5.75cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^1$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west,
%skip coords between index={7}{8}
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/bilaplace_penalty_9patches_matching_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/bilaplace_penalty_9patches_matching_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

%	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_non_matching_no_proj_breitenberger_SIMPLE_ILU_p4.txt};
%    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/bilaplace_penalty_9patches_matching_josef_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/bilaplace_penalty_9patches_matching_josef_p3.txt};
    \addlegendentry{$p=3$ scaled};

%	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_non_matching_no_proj_SIMPLE_ILU_p4.txt};
%    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/bilaplace_penalty_9patches_matching_proj_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/bilaplace_penalty_9patches_matching_proj_p3.txt};
    \addlegendentry{$p=3$ proj};

%	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_non_matching_proj_SIMPLE_ILU_p4.txt};
%    \addlegendentry{$p=4$ proj};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.415}{2}{black};
\logLogSlopeReverseTriangle{0.795}{0.08}{0.065}{3}{black};
%\logLogSlopeReverseTriangle{0.54}{0.08}{0.065}{3}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_bilaplace_9patches_conforming_h2.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.775\textwidth,
height=5.75cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^2$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west,
%skip coords between index={7}{8}
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_9patches_matching_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_9patches_matching_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

%	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_non_matching_no_proj_breitenberger_SIMPLE_ILU_p4.txt};
%    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_9patches_matching_josef_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_9patches_matching_josef_p3.txt};
    \addlegendentry{$p=3$ scaled};

%	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_non_matching_no_proj_SIMPLE_ILU_p4.txt};
%    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_9patches_matching_proj_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_9patches_matching_proj_p3.txt};
    \addlegendentry{$p=3$ proj};

%	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_non_matching_proj_SIMPLE_ILU_p4.txt};
%    \addlegendentry{$p=4$ proj};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.505}{1}{black};
\logLogSlopeReverseTriangle{0.795}{0.08}{0.065}{2}{black};
%\logLogSlopeReverseTriangle{0.54}{0.08}{0.065}{3}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_bilaplace_9patches_conforming_l2.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.775\textwidth,
height=5.75cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $L^2$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west,
%skip coords between index={7}{8}
]


	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/bilaplace_penalty_9patches_matching_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/bilaplace_penalty_9patches_matching_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

%	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_non_matching_no_proj_breitenberger_SIMPLE_ILU_p4.txt};
%    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/bilaplace_penalty_9patches_matching_josef_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/bilaplace_penalty_9patches_matching_josef_p3.txt};
    \addlegendentry{$p=3$ scaled};

%	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_non_matching_no_proj_SIMPLE_ILU_p4.txt};
%    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/bilaplace_penalty_9patches_matching_proj_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/bilaplace_penalty_9patches_matching_proj_p3.txt};
    \addlegendentry{$p=3$ proj};

%	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_non_matching_proj_SIMPLE_ILU_p4.txt};
%    \addlegendentry{$p=4$ proj};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};


{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.49}{2}{black};
\logLogSlopeReverseTriangle{0.795}{0.08}{0.065}{4}{black};
%\logLogSlopeReverseTriangle{0.54}{0.08}{0.065}{3}{black};
}

\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_bilaplace_conforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^2$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_tilted_coupling_2patches_conforming_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_tilted_coupling_2patches_conforming_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_tilted_coupling_2patches_conforming_breitenberger_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_tilted_coupling_2patches_conforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_tilted_coupling_2patches_conforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_tilted_coupling_2patches_conforming_p4.txt};
    \addlegendentry{$p=4$ scaled};

%    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_tilted_coupling_2patches_conforming_p4.txt};
%    \addlegendentry{$p=4$};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_tilted_coupling_2patches_conforming_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_tilted_coupling_2patches_conforming_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_tilted_coupling_2patches_conforming_projected_p4.txt};
    \addlegendentry{$p=4$ proj};

%    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_tilted_coupling_2patches_conforming_projected_p4.txt};
%    \addlegendentry{$p=4, p^{red}=2$};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.64}{1}{black};
\logLogSlopeReverseTriangle{0.85}{0.08}{0.315}{2}{black};
\logLogSlopeReverseTriangle{0.85}{0.08}{0.058}{3}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_bilaplace_curved_conforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^2$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west
]
	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_curved_coupling_2patches_conforming_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_curved_coupling_2patches_conforming_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_curved_coupling_2patches_conforming_breitenberger_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_curved_coupling_2patches_conforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_curved_coupling_2patches_conforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_curved_coupling_2patches_conforming_p4.txt};
    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_curved_coupling_2patches_conforming_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_curved_coupling_2patches_conforming_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_curved_coupling_2patches_conforming_projected_p4.txt};
    \addlegendentry{$p=4$ proj};

%    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_tilted_coupling_2patches_conforming_projected_p4.txt};
%    \addlegendentry{$p=4, p^{red}=2$};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.61}{1}{black};
\logLogSlopeReverseTriangle{0.82}{0.08}{0.34}{2}{black};
\logLogSlopeReverseTriangle{0.82}{0.08}{0.06}{3}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_bilaplace_curved_nonconforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^2$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west
]


	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_curved_coupling_2patches_nonconforming_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_curved_coupling_2patches_nonconforming_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_curved_coupling_2patches_nonconforming_breitenberger_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_curved_coupling_2patches_nonconforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_curved_coupling_2patches_nonconforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_curved_coupling_2patches_nonconforming_p4.txt};
    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_curved_coupling_2patches_nonconforming_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_curved_coupling_2patches_nonconforming_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_curved_coupling_2patches_nonconforming_projected_p4.txt};
    \addlegendentry{$p=4$ proj};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.615}{1}{black};
\logLogSlopeReverseTriangle{0.8}{0.08}{0.35}{2}{black};
\logLogSlopeReverseTriangle{0.8}{0.08}{0.08}{3}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_bilaplace_curved_nonconforming_h1_ilu.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^1$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west,
skip coords between index={6}{7}
]


	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/bilaplace_penalty_non_matching_no_proj_breitenberger_SIMPLE_ILU_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/bilaplace_penalty_non_matching_no_proj_breitenberger_SIMPLE_ILU_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/bilaplace_penalty_non_matching_no_proj_breitenberger_SIMPLE_ILU_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/bilaplace_penalty_non_matching_no_proj_SIMPLE_ILU_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/bilaplace_penalty_non_matching_no_proj_SIMPLE_ILU_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/bilaplace_penalty_non_matching_no_proj_SIMPLE_ILU_p4.txt};
    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/bilaplace_penalty_non_matching_proj_SIMPLE_ILU_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/bilaplace_penalty_non_matching_proj_SIMPLE_ILU_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/bilaplace_penalty_non_matching_proj_SIMPLE_ILU_p4.txt};
    \addlegendentry{$p=4$ proj};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};


{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.415}{2}{black};
\logLogSlopeReverseTriangle{0.85}{0.08}{0.13}{3}{black};
\logLogSlopeReverseTriangle{0.65}{0.08}{0.065}{4}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_bilaplace_curved_nonconforming_h2_ilu.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^2$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west,
skip coords between index={7}{8}
]


	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_non_matching_no_proj_breitenberger_SIMPLE_ILU_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_non_matching_no_proj_breitenberger_SIMPLE_ILU_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_non_matching_no_proj_breitenberger_SIMPLE_ILU_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_non_matching_no_proj_SIMPLE_ILU_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_non_matching_no_proj_SIMPLE_ILU_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_non_matching_no_proj_SIMPLE_ILU_p4.txt};
    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_non_matching_proj_SIMPLE_ILU_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_non_matching_proj_SIMPLE_ILU_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/bilaplace_penalty_non_matching_proj_SIMPLE_ILU_p4.txt};
    \addlegendentry{$p=4$ proj};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};


{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.55}{1}{black};
\logLogSlopeReverseTriangle{0.85}{0.08}{0.095}{2}{black};
\logLogSlopeReverseTriangle{0.54}{0.08}{0.065}{3}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_bilaplace_curved_nonconforming_ilu_condest.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=2*1e3,
xminorticks=true,
ymode=log,
%ymin=8e-1,
%ymax=2,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Condition number,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend style={at={(0.9,0.3)},anchor=east},
%legend pos= north east,
%skip coords between index={7}{8}
]

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 6] {\dataDir/bilaplace_penalty_non_matching_proj_SIMPLE_ILU_condest_p2.txt};
    \addlegendentry{$p=2$, ILU};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 6] {\dataDir/bilaplace_penalty_non_matching_proj_SIMPLE_ILU_condest_p3.txt};
    \addlegendentry{$p=3$, ILU};

    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 6] {\dataDir/bilaplace_penalty_non_matching_proj_SIMPLE_ILU_condest_p4.txt};
    \addlegendentry{$p=4$, ILU};

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 6] {\dataDir/bilaplace_penalty_non_matching_proj_SIMPLE_SIMPLE_condest_p2.txt};
    \addlegendentry{$p=2$, SIMPLE};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 6] {\dataDir/bilaplace_penalty_non_matching_proj_SIMPLE_SIMPLE_condest_p3.txt};
    \addlegendentry{$p=3$, SIMPLE};

    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 6] {\dataDir/bilaplace_penalty_non_matching_proj_SIMPLE_SIMPLE_condest_p4.txt};
    \addlegendentry{$p=4$, SIMPLE};


%\logLogSlopeReverseTriangle{0.85}{0.08}{0.445}{2}{black};
%\logLogSlopeReverseTriangle{0.85}{0.08}{0.25}{3}{black};
%\logLogSlopeReverseTriangle{0.85}{0.08}{0.0625}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};

\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_bilaplace_curved_nonconforming_l2_ilu.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $L^2$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west,
skip coords between index={6}{7}
]


	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/bilaplace_penalty_non_matching_no_proj_breitenberger_SIMPLE_ILU_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/bilaplace_penalty_non_matching_no_proj_breitenberger_SIMPLE_ILU_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/bilaplace_penalty_non_matching_no_proj_breitenberger_SIMPLE_ILU_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/bilaplace_penalty_non_matching_no_proj_SIMPLE_ILU_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/bilaplace_penalty_non_matching_no_proj_SIMPLE_ILU_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/bilaplace_penalty_non_matching_no_proj_SIMPLE_ILU_p4.txt};
    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/bilaplace_penalty_non_matching_proj_SIMPLE_ILU_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/bilaplace_penalty_non_matching_proj_SIMPLE_ILU_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/bilaplace_penalty_non_matching_proj_SIMPLE_ILU_p4.txt};
    \addlegendentry{$p=4$ proj};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};


{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.385}{2}{black};
\logLogSlopeReverseTriangle{0.85}{0.08}{0.125}{3}{black};
\logLogSlopeReverseTriangle{0.615}{0.08}{0.065}{4}{black};%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_bilaplace_curved_nonconforming_no_precond_condest.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Condition number,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= north west,
%skip coords between index={7}{8}
]

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 6] {\dataDir/bilaplace_penalty_non_matching_proj_NO_PRECOND_condest_p2.txt};
    \addlegendentry{$p=2, p^{red}=0$};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 6] {\dataDir/bilaplace_penalty_non_matching_proj_NO_PRECOND_condest_p3.txt};
    \addlegendentry{$p=3, p^{red}=1$};

    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 6] {\dataDir/bilaplace_penalty_non_matching_proj_NO_PRECOND_condest_p4.txt};
    \addlegendentry{$p=4, p^{red}=2$};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};



\logLogSlopeTriangle{0.9}{0.08}{0.51}{5}{black};
\logLogSlopeTriangle{0.9}{0.08}{0.66}{6}{black};
\logLogSlopeTriangle{0.9}{0.08}{0.82}{7}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};

\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_bilaplace_diagonal_trimmed_nonconforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
xmax=1.5e2,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^2$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/bilaplace_coupling_trimmed_diagonal_nonConforming_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/bilaplace_coupling_trimmed_diagonal_nonConforming_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/bilaplace_coupling_trimmed_diagonal_nonConforming_breitenberger_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/bilaplace_coupling_trimmed_diagonal_nonConforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/bilaplace_coupling_trimmed_diagonal_nonConforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/bilaplace_coupling_trimmed_diagonal_nonConforming_p4.txt};
    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/bilaplace_coupling_trimmed_diagonal_nonConforming_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/bilaplace_coupling_trimmed_diagonal_nonConforming_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/bilaplace_coupling_trimmed_diagonal_nonConforming_projected_p4.txt};
    \addlegendentry{$p=4$ proj};

{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.605}{1}{black};
\logLogSlopeReverseTriangle{0.85}{0.08}{0.22}{2}{black};
\logLogSlopeReverseTriangle{0.65}{0.08}{0.06}{3}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_bilaplace_diagonal_trimmed_nonconforming_h1.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
xmax=1.5e2,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^1$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/bilaplace_coupling_trimmed_diagonal_nonConforming_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/bilaplace_coupling_trimmed_diagonal_nonConforming_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/bilaplace_coupling_trimmed_diagonal_nonConforming_breitenberger_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/bilaplace_coupling_trimmed_diagonal_nonConforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/bilaplace_coupling_trimmed_diagonal_nonConforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/bilaplace_coupling_trimmed_diagonal_nonConforming_p4.txt};
    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/bilaplace_coupling_trimmed_diagonal_nonConforming_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/bilaplace_coupling_trimmed_diagonal_nonConforming_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/bilaplace_coupling_trimmed_diagonal_nonConforming_projected_p4.txt};
    \addlegendentry{$p=4$ proj};



{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.435}{2}{black};
\logLogSlopeReverseTriangle{0.85}{0.08}{0.135}{3}{black};
\logLogSlopeReverseTriangle{0.64}{0.08}{0.055}{4}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_bilaplace_diagonal_trimmed_nonconforming_l2.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
xmax=1.5e2,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $L^2$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_coupling_trimmed_diagonal_nonConforming_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_coupling_trimmed_diagonal_nonConforming_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_coupling_trimmed_diagonal_nonConforming_breitenberger_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_coupling_trimmed_diagonal_nonConforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_coupling_trimmed_diagonal_nonConforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_coupling_trimmed_diagonal_nonConforming_p4.txt};
    \addlegendentry{$p=4$ scaled};

%    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_tilted_coupling_2patches_conforming_p4.txt};
%    \addlegendentry{$p=4$};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_coupling_trimmed_diagonal_nonConforming_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_coupling_trimmed_diagonal_nonConforming_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_coupling_trimmed_diagonal_nonConforming_projected_p4.txt};
    \addlegendentry{$p=4$ proj};

%    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_tilted_coupling_2patches_conforming_projected_p4.txt};
%    \addlegendentry{$p=4, p^{red}=2$};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.435}{2}{black};
\logLogSlopeReverseTriangle{0.835}{0.08}{0.135}{4}{black};
\logLogSlopeReverseTriangle{0.64}{0.08}{0.055}{5}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_bilaplace_nonconforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^2$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_tilted_coupling_2patches_nonconforming_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_tilted_coupling_2patches_nonconforming_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_tilted_coupling_2patches_nonconforming_breitenberger_p4.txt};
    \addlegendentry{$p=4$};


	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_tilted_coupling_2patches_nonconforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_tilted_coupling_2patches_nonconforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_tilted_coupling_2patches_nonconforming_p4.txt};
    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_tilted_coupling_2patches_nonconforming_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_tilted_coupling_2patches_nonconforming_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_tilted_coupling_2patches_nonconforming_projected_p4.txt};
    \addlegendentry{$p=4$ proj};

%    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/laplace_coupling_2patches_nonconforming_projected_p4.txt};
%    \addlegendentry{$p=4, p^{red}=2$};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.63}{1}{black};
\logLogSlopeReverseTriangle{0.85}{0.08}{0.3}{2}{black};
\logLogSlopeReverseTriangle{0.85}{0.08}{0.055}{3}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_bilaplace_trimmed_conforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^2$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/bilaplace_trimmed_coupling_2patches_conforming_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/bilaplace_trimmed_coupling_2patches_conforming_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/bilaplace_trimmed_coupling_2patches_conforming_breitenberger_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/bilaplace_trimmed_coupling_2patches_conforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/bilaplace_trimmed_coupling_2patches_conforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/bilaplace_trimmed_coupling_2patches_conforming_p4.txt};
    \addlegendentry{$p=4$ scaled};

%    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_tilted_coupling_2patches_conforming_p4.txt};
%    \addlegendentry{$p=4$};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/bilaplace_trimmed_coupling_2patches_conforming_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/bilaplace_trimmed_coupling_2patches_conforming_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/bilaplace_trimmed_coupling_2patches_conforming_projected_p4.txt};
    \addlegendentry{$p=4$ proj};

%    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_tilted_coupling_2patches_conforming_projected_p4.txt};
%    \addlegendentry{$p=4, p^{red}=2$};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.64}{1}{black};
\logLogSlopeReverseTriangle{0.85}{0.08}{0.33}{2}{black};
\logLogSlopeReverseTriangle{0.835}{0.08}{0.055}{3}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_conditioning_bilaplace_conforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Condition number,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= outer north east,
legend style={cells={align=left}}
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_tilted_coupling_2patches_conforming_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_tilted_coupling_2patches_conforming_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_tilted_coupling_2patches_conforming_breitenberger_p4.txt};
    \addlegendentry{$p=4$};


	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_tilted_coupling_2patches_conforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_tilted_coupling_2patches_conforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_tilted_coupling_2patches_conforming_p4.txt};
    \addlegendentry{$p=4$ scaled};


	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_tilted_coupling_2patches_conforming_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_tilted_coupling_2patches_conforming_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_tilted_coupling_2patches_conforming_projected_p4.txt};
    \addlegendentry{$p=4$ proj};


	\addplot [color=black, solid]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_coupling_1patch_p2.txt};
    \addlegendentry{$p=2$ single\\ patch};
	
	\addplot[color=black, dotted] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_coupling_1patch_p3.txt};
    \addlegendentry{$p=3$ single\\ patch};

	\addplot[color=black, dashed] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_coupling_1patch_p4.txt};
    \addlegendentry{$p=4$ single\\ patch};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
%\logLogSlopeReverseTriangle{0.85}{0.08}{0.47}{2}{black};
%\logLogSlopeReverseTriangle{0.85}{0.08}{0.245}{3}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}

\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_conditioning_bilaplace_curved_conforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Condition number,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= outer north east,
legend style={cells={align=left}}
]
	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_curved_coupling_2patches_conforming_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_curved_coupling_2patches_conforming_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_curved_coupling_2patches_conforming_breitenberger_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_curved_coupling_2patches_conforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_curved_coupling_2patches_conforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_curved_coupling_2patches_conforming_p4.txt};
    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_curved_coupling_2patches_conforming_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_curved_coupling_2patches_conforming_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_curved_coupling_2patches_conforming_projected_p4.txt};
    \addlegendentry{$p=4$ proj};

	\addplot [color=black, dashed]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_coupling_1patch_p2.txt};
    \addlegendentry{$p=2$ single\\ patch};
	
	\addplot[color=black, dotted] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_coupling_1patch_p3.txt};
    \addlegendentry{$p=3$ single\\ patch};

	\addplot[color=black, dotted] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_coupling_1patch_p4.txt};
    \addlegendentry{$p=4$ single\\ patch};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
%\logLogSlopeReverseTriangle{0.85}{0.08}{0.47}{2}{black};
%\logLogSlopeReverseTriangle{0.85}{0.08}{0.245}{3}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}

\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_conditioning_bilaplace_curved_nonconforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Condition number,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos=outer north east,
legend style={cells={align=left}}
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_curved_coupling_2patches_nonconforming_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_curved_coupling_2patches_nonconforming_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_curved_coupling_2patches_nonconforming_breitenberger_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_curved_coupling_2patches_nonconforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_curved_coupling_2patches_nonconforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_curved_coupling_2patches_nonconforming_p4.txt};
    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_curved_coupling_2patches_nonconforming_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_curved_coupling_2patches_nonconforming_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_curved_coupling_2patches_nonconforming_projected_p4.txt};
    \addlegendentry{$p=4$ proj};

	\addplot [color=black, dashed]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_coupling_1patch_p2.txt};
    \addlegendentry{$p=2$ single\\ patch};
	
	\addplot[color=black, dotted] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_coupling_1patch_p3.txt};
    \addlegendentry{$p=3$ single\\ patch};

	\addplot[color=black, dotted] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_coupling_1patch_p4.txt};
    \addlegendentry{$p=4$ single\\ patch};

%    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/laplace_coupling_2patches_nonconforming_projected_p4.txt};
%    \addlegendentry{$p=4, p^{red}=2$};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
%\logLogSlopeReverseTriangle{0.85}{0.08}{0.47}{2}{black};
%\logLogSlopeReverseTriangle{0.85}{0.08}{0.245}{3}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}

\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_conditioning_bilaplace_diagonal_trimmed_nonconforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
xmax=1.5e2,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Condition number,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= outer north east,
legend style={cells={align=left}}
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_coupling_trimmed_diagonal_nonConforming_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_coupling_trimmed_diagonal_nonConforming_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_coupling_trimmed_diagonal_nonConforming_breitenberger_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_coupling_trimmed_diagonal_nonConforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_coupling_trimmed_diagonal_nonConforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_coupling_trimmed_diagonal_nonConforming_p4.txt};
    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_coupling_trimmed_diagonal_nonConforming_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_coupling_trimmed_diagonal_nonConforming_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_coupling_trimmed_diagonal_nonConforming_projected_p4.txt};
    \addlegendentry{$p=4$ proj};


\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_conditioning_bilaplace_nonconforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Condition number,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= outer north east,
legend style={cells={align=left}}
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_tilted_coupling_2patches_nonconforming_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_tilted_coupling_2patches_nonconforming_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_tilted_coupling_2patches_nonconforming_breitenberger_p4.txt};
    \addlegendentry{$p=4$};


	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_tilted_coupling_2patches_nonconforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_tilted_coupling_2patches_nonconforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_tilted_coupling_2patches_nonconforming_p4.txt};
    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_tilted_coupling_2patches_nonconforming_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_tilted_coupling_2patches_nonconforming_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_tilted_coupling_2patches_nonconforming_projected_p4.txt};
    \addlegendentry{$p=4$ proj};

	\addplot [color=black, dashed]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_coupling_1patch_p2.txt};
    \addlegendentry{$p=2$ single\\ patch};
	
	\addplot[color=black, dotted] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_coupling_1patch_p3.txt};
    \addlegendentry{$p=3$ single\\ patch};

	\addplot[color=black, dotted] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_coupling_1patch_p4.txt};
    \addlegendentry{$p=4$ single\\ patch};
    
%    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/laplace_coupling_2patches_nonconforming_projected_p4.txt};
%    \addlegendentry{$p=4, p^{red}=2$};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
%\logLogSlopeTriangle{0.85}{0.15}{0.42}{5}{black};
%\logLogSlopeTriangle{0.85}{0.15}{0.285}{3}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}

\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_conditioning_bilaplace_trimmed_conforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Condition number,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= outer north east,
legend style={cells={align=left}}
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_trimmed_coupling_2patches_conforming_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_trimmed_coupling_2patches_conforming_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_trimmed_coupling_2patches_conforming_breitenberger_p4.txt};
    \addlegendentry{$p=4$};


	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_trimmed_coupling_2patches_conforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_trimmed_coupling_2patches_conforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_trimmed_coupling_2patches_conforming_p4.txt};
    \addlegendentry{$p=4$ scaled};


	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_trimmed_coupling_2patches_conforming_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_trimmed_coupling_2patches_conforming_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_trimmed_coupling_2patches_conforming_projected_p4.txt};
    \addlegendentry{$p=4$ proj};


%	\addplot [color=black, solid]
%    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_coupling_1patch_p2.txt};
%    \addlegendentry{$p=2$ single\\ patch};
%	
%	\addplot[color=black, dotted] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_coupling_1patch_p3.txt};
%    \addlegendentry{$p=3$ single\\ patch};
%
%	\addplot[color=black, dashed] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_coupling_1patch_p4.txt};
%    \addlegendentry{$p=4$ single\\ patch};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
%\logLogSlopeReverseTriangle{0.85}{0.08}{0.47}{2}{black};
%\logLogSlopeReverseTriangle{0.85}{0.08}{0.245}{3}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}

\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_conditioning_laplace_conforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Condition number,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south east
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/laplace_coupling_2patches_conforming_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/laplace_coupling_2patches_conforming_p3.txt};
    \addlegendentry{$p=3$};


    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/laplace_coupling_2patches_conforming_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/laplace_coupling_2patches_conforming_projected_p2.txt};
    \addlegendentry{$p=2, p^{red}=0$};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/laplace_coupling_2patches_conforming_projected_p3.txt};
    \addlegendentry{$p=3, p^{red}=1$};

    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/laplace_coupling_2patches_conforming_projected_p4.txt};
    \addlegendentry{$p=4, p^{red}=2$};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
%\logLogSlopeReverseTriangle{0.85}{0.08}{0.47}{2}{black};
%\logLogSlopeReverseTriangle{0.85}{0.08}{0.245}{3}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}

\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_conditioning_laplace_curved_conforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Condition number,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south east
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/laplace_coupling_2patches_conforming_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/laplace_coupling_2patches_conforming_p3.txt};
    \addlegendentry{$p=3$};


%    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/laplace_coupling_2patches_conforming_p4.txt};
%    \addlegendentry{$p=4$};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/laplace_coupling_2patches_conforming_projected_p2.txt};
    \addlegendentry{$p=2, p^{red}=0$};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/laplace_coupling_2patches_conforming_projected_p3.txt};
    \addlegendentry{$p=3, p^{red}=1$};

%    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/laplace_coupling_2patches_conforming_projected_p4.txt};
%    \addlegendentry{$p=4, p^{red}=2$};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
%\logLogSlopeReverseTriangle{0.85}{0.08}{0.47}{2}{black};
%\logLogSlopeReverseTriangle{0.85}{0.08}{0.245}{3}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}

\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_conditioning_laplace_curved_nonconforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Condition number,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south east
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/laplace_curved_coupling_2patches_nonconforming_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/laplace_curved_coupling_2patches_nonconforming_p3.txt};
    \addlegendentry{$p=3$};


%    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/laplace_coupling_2patches_nonconforming_p4.txt};
%    \addlegendentry{$p=4$};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/laplace_curved_coupling_2patches_nonconforming_projected_p2.txt};
    \addlegendentry{$p=2, p^{red}=0$};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/laplace_curved_coupling_2patches_nonconforming_projected_p3.txt};
    \addlegendentry{$p=3, p^{red}=1$};

%    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/laplace_coupling_2patches_nonconforming_projected_p4.txt};
%    \addlegendentry{$p=4, p^{red}=2$};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
%\logLogSlopeReverseTriangle{0.85}{0.08}{0.47}{2}{black};
%\logLogSlopeReverseTriangle{0.85}{0.08}{0.245}{3}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}

\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_conditioning_laplace_nonconforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Condition number,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south east
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/laplace_coupling_2patches_nonconforming_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/laplace_coupling_2patches_nonconforming_p3.txt};
    \addlegendentry{$p=3$};


%    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/laplace_coupling_2patches_nonconforming_p4.txt};
%    \addlegendentry{$p=4$};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/laplace_coupling_2patches_nonconforming_projected_p2.txt};
    \addlegendentry{$p=2, p^{red}=0$};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/laplace_coupling_2patches_nonconforming_projected_p3.txt};
    \addlegendentry{$p=3, p^{red}=1$};

%    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/laplace_coupling_2patches_nonconforming_projected_p4.txt};
%    \addlegendentry{$p=4, p^{red}=2$};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
%\logLogSlopeReverseTriangle{0.85}{0.08}{0.47}{2}{black};
%\logLogSlopeReverseTriangle{0.85}{0.08}{0.245}{3}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}

\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_conditioning_laplace_trimmed_conforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Condition number,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos=outer north east
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/laplace_trimmed_coupling_2patches_conforming_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/laplace_trimmed_coupling_2patches_conforming_p3.txt};
    \addlegendentry{$p=3$};


    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/laplace_trimmed_coupling_2patches_conforming_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/laplace_trimmed_coupling_2patches_conforming_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/laplace_trimmed_coupling_2patches_conforming_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/laplace_trimmed_coupling_2patches_conforming_projected_p4.txt};
    \addlegendentry{$p=4$ proj};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
%\logLogSlopeReverseTriangle{0.85}{0.08}{0.47}{2}{black};
%\logLogSlopeReverseTriangle{0.85}{0.08}{0.245}{3}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}

\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_conditioning_shell_curved_conforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Condition number,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= outer north east,
legend style={cells={align=left}}
]
	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_curved_coupling_2patches_conforming_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_curved_coupling_2patches_conforming_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_curved_coupling_2patches_conforming_breitenberger_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_curved_coupling_2patches_conforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_curved_coupling_2patches_conforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_curved_coupling_2patches_conforming_p4.txt};
    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_curved_coupling_2patches_conforming_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_curved_coupling_2patches_conforming_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_curved_coupling_2patches_conforming_projected_p4.txt};
    \addlegendentry{$p=4$ proj};

%	\addplot [color=black, dashed]
%    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_coupling_1patch_p2.txt};
%    \addlegendentry{$p=2$ single\\ patch};
%	
%	\addplot[color=black, dotted] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_coupling_1patch_p3.txt};
%    \addlegendentry{$p=3$ single\\ patch};
%
%	\addplot[color=black, dotted] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_coupling_1patch_p4.txt};
%    \addlegendentry{$p=4$ single\\ patch};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
%\logLogSlopeReverseTriangle{0.85}{0.08}{0.47}{2}{black};
%\logLogSlopeReverseTriangle{0.85}{0.08}{0.245}{3}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}

\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_conditioning_shell_curved_cut_trimmed_conforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1.5e2,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Condition number,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= outer north east,
legend style={cells={align=left}},
skip coords between index={0}{1}
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/shell_trimmed_curved_cut_2patches_fromFile_breitenberger_conforming_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/shell_trimmed_curved_cut_2patches_fromFile_breitenberger_conforming_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/shell_trimmed_curved_cut_2patches_fromFile_breitenberger_conforming_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/shell_trimmed_curved_cut_2patches_fromFile_conforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/shell_trimmed_curved_cut_2patches_fromFile_conforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/shell_trimmed_curved_cut_2patches_fromFile_conforming_p4.txt};
    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/shell_trimmed_curved_cut_coupling_2patches_projected_conforming_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/shell_trimmed_curved_cut_coupling_2patches_projected_conforming_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/shell_trimmed_curved_cut_coupling_2patches_projected_conforming_p4.txt};
    \addlegendentry{$p=4$ proj};



\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_conditioning_shell_curved_cut_trimmed_nonconforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
xmax=1.e2,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Condition number,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= outer north east,
legend style={cells={align=left}},
skip coords between index={5}{6}
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/shell_trimmed_curved_cut_2patches_breitenberger_nonConforming_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/shell_trimmed_curved_cut_2patches_breitenberger_nonConforming_p3.txt};
    \addlegendentry{$p=3$};

%	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/shell_trimmed_curved_cut_2patches_breitenberger_nonConforming_p4.txt};
%    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/shell_trimmed_curved_cut_2patches_nonConforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/shell_trimmed_curved_cut_2patches_nonConforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

%	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/shell_trimmed_curved_cut_2patches_nonConforming_p4.txt};
%    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/shell_trimmed_curved_cut_coupling_2patches_projected_nonConforming_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/shell_trimmed_curved_cut_coupling_2patches_projected_nonConforming_p3.txt};
    \addlegendentry{$p=3$ proj};

%	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 3] {\dataDir/shell_trimmed_curved_cut_coupling_2patches_projected_nonConforming_p4.txt};
%    \addlegendentry{$p=4$ proj};



\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_conditioning_shell_curved_nonconforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Condition number,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos=outer north east,
legend style={cells={align=left}}
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_curved_coupling_2patches_nonconforming_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_curved_coupling_2patches_nonconforming_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_curved_coupling_2patches_nonconforming_breitenberger_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_curved_coupling_2patches_nonconforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_curved_coupling_2patches_nonconforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_curved_coupling_2patches_nonconforming_p4.txt};
    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_curved_coupling_2patches_nonconforming_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_curved_coupling_2patches_nonconforming_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_curved_coupling_2patches_nonconforming_projected_p4.txt};
    \addlegendentry{$p=4$ proj};

%	\addplot [color=black, dashed]
%    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_coupling_1patch_p2.txt};
%    \addlegendentry{$p=2$ single\\ patch};
%	
%	\addplot[color=black, dotted] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_coupling_1patch_p3.txt};
%    \addlegendentry{$p=3$ single\\ patch};
%
%	\addplot[color=black, dotted] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/bilaplace_coupling_1patch_p4.txt};
%    \addlegendentry{$p=4$ single\\ patch};

%    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/laplace_coupling_2patches_nonconforming_projected_p4.txt};
%    \addlegendentry{$p=4, p^{red}=2$};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
%\logLogSlopeReverseTriangle{0.85}{0.08}{0.47}{2}{black};
%\logLogSlopeReverseTriangle{0.85}{0.08}{0.245}{3}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}

\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_conditioning_shell_diagonal_trimmed_conforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1.5e2,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Condition number,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= outer north east,
legend style={cells={align=left}}
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_coupling_trimmed_diagonal_conforming_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_coupling_trimmed_diagonal_conforming_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_coupling_trimmed_diagonal_conforming_breitenberger_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_coupling_trimmed_diagonal_conforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_coupling_trimmed_diagonal_conforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_coupling_trimmed_diagonal_conforming_p4.txt};
    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_coupling_trimmed_diagonal_conforming_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_coupling_trimmed_diagonal_conforming_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_coupling_trimmed_diagonal_conforming_projected_p4.txt};
    \addlegendentry{$p=4$ proj};


\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_conditioning_shell_diagonal_trimmed_nonconforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1.5e2,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Condition number,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= outer north east,
legend style={cells={align=left}}
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_coupling_trimmed_diagonal_nonConforming_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_coupling_trimmed_diagonal_nonConforming_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_coupling_trimmed_diagonal_nonConforming_breitenberger_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_coupling_trimmed_diagonal_nonConforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_coupling_trimmed_diagonal_nonConforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_coupling_trimmed_diagonal_nonConforming_p4.txt};
    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_coupling_trimmed_diagonal_nonConforming_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_coupling_trimmed_diagonal_nonConforming_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_coupling_trimmed_diagonal_nonConforming_projected_p4.txt};
    \addlegendentry{$p=4$ proj};


\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_conditioning_shell_trimmed_conforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Condition number,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= outer north east,
legend style={cells={align=left}}
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_trimmed_coupling_2patches_fromFile_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_trimmed_coupling_2patches_fromFile_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_trimmed_coupling_2patches_fromFile_breitenberger_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_trimmed_coupling_2patches_fromFile_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_trimmed_coupling_2patches_fromFile_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_trimmed_coupling_2patches_fromFile_p4.txt};
    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_trimmed_coupling_2patches_fromFile_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_trimmed_coupling_2patches_fromFile_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_trimmed_coupling_2patches_fromFile_projected_p4.txt};
    \addlegendentry{$p=4$ proj};


\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_conditioning_shell_trimmed_nonconforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Condition number,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= outer north east,
legend style={cells={align=left}}
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_trimmed_coupling_2patches_fromFile_breitenberger_nonConforming_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_trimmed_coupling_2patches_fromFile_breitenberger_nonConforming_p3.txt};
    \addlegendentry{$p=3$};

%	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_trimmed_coupling_2patches_fromFile_breitenberger_nonConforming_p4.txt};
%    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_trimmed_coupling_2patches_fromFile_nonConforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_trimmed_coupling_2patches_fromFile_nonConforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

%	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_trimmed_coupling_2patches_fromFile_nonConforming_p4.txt};
%    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_trimmed_coupling_2patches_fromFile_projected_nonConforming_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_trimmed_coupling_2patches_fromFile_projected_nonConforming_p3.txt};
    \addlegendentry{$p=3$ proj};

%	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 4] {\dataDir/shell_trimmed_coupling_2patches_fromFile_projected_nonConforming_p4.txt};
%    \addlegendentry{$p=4$ proj};


\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_laplace_conforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^1$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/laplace_coupling_2patches_conforming_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/laplace_coupling_2patches_conforming_p3.txt};
    \addlegendentry{$p=3$};


    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/laplace_coupling_2patches_conforming_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/laplace_coupling_2patches_conforming_projected_p2.txt};
    \addlegendentry{$p=2, p^{red}=0$};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/laplace_coupling_2patches_conforming_projected_p3.txt};
    \addlegendentry{$p=3, p^{red}=1$};

    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/laplace_coupling_2patches_conforming_projected_p4.txt};
    \addlegendentry{$p=4, p^{red}=2$};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.47}{2}{black};
\logLogSlopeReverseTriangle{0.85}{0.08}{0.245}{3}{black};
\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_laplace_curved_conforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
xmax=1e2,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^1$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/laplace_curved_coupling_2patches_conforming_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/laplace_curved_coupling_2patches_conforming_p3.txt};
    \addlegendentry{$p=3$};


%    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/laplace_curved_coupling_2patches_conforming_p4.txt};
%    \addlegendentry{$p=4$};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/laplace_curved_coupling_2patches_conforming_projected_p2.txt};
    \addlegendentry{$p=2, p^{red}=0$};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/laplace_curved_coupling_2patches_conforming_projected_p3.txt};
    \addlegendentry{$p=3, p^{red}=1$};

%    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/laplace_curved_coupling_2patches_conforming_projected_p4.txt};
%    \addlegendentry{$p=4, p^{red}=2$};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.325}{2}{black};
\logLogSlopeReverseTriangle{0.8}{0.08}{0.065}{3}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_laplace_curved_nonconforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^1$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/laplace_curved_coupling_2patches_nonconforming_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/laplace_curved_coupling_2patches_nonconforming_p3.txt};
    \addlegendentry{$p=3$};


%    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/laplace_coupling_2patches_nonconforming_p4.txt};
%    \addlegendentry{$p=4$};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/laplace_curved_coupling_2patches_nonconforming_projected_p2.txt};
    \addlegendentry{$p=2, p^{red}=0$};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/laplace_curved_coupling_2patches_nonconforming_projected_p3.txt};
    \addlegendentry{$p=3, p^{red}=1$};

%    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/laplace_coupling_2patches_nonconforming_projected_p4.txt};
%    \addlegendentry{$p=4, p^{red}=2$};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.335}{2}{black};
\logLogSlopeReverseTriangle{0.82}{0.08}{0.0625}{3}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_laplace_curved_nonconforming_fd.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^1$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west,
skip coords between index={7}{8}
]


	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{3}^0.5, y index = 1] {\dataDir/laplace_penalty_non_matching_no_proj_SIMPLE_FD_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 1] {\dataDir/laplace_penalty_non_matching_no_proj_SIMPLE_FD_p3.txt};
    \addlegendentry{$p=3$};

    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 1] {\dataDir/laplace_penalty_non_matching_no_proj_SIMPLE_FD_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{3}^0.5, y index = 1] {\dataDir/laplace_penalty_non_matching_proj_SIMPLE_FD_p2.txt};
    \addlegendentry{$p=2, p^{red}=0$};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 1] {\dataDir/laplace_penalty_non_matching_proj_SIMPLE_FD_p3.txt};
    \addlegendentry{$p=3, p^{red}=1$};

    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 1] {\dataDir/laplace_penalty_non_matching_proj_SIMPLE_FD_p4.txt};
    \addlegendentry{$p=4, p^{red}=2$};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.445}{2}{black};
\logLogSlopeReverseTriangle{0.85}{0.08}{0.25}{3}{black};
\logLogSlopeReverseTriangle{0.85}{0.08}{0.0625}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_laplace_curved_nonconforming_fd_condest.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=2*1e3,
xminorticks=true,
ymode=log,
%ymin=8e-1,
%ymax=2,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Condition number,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend style={at={(0.9,0.3)},anchor=east},
%legend pos= north east,
%skip coords between index={7}{8}
]

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{3}^0.5, y index = 5] {\dataDir/laplace_penalty_non_matching_proj_SIMPLE_FD_condest_p2.txt};
    \addlegendentry{$p=2$, FD};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 5] {\dataDir/laplace_penalty_non_matching_proj_SIMPLE_FD_condest_p3.txt};
    \addlegendentry{$p=3$, FD};

    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 5] {\dataDir/laplace_penalty_non_matching_proj_SIMPLE_FD_condest_p4.txt};
    \addlegendentry{$p=4$, FD};

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{3}^0.5, y index = 5] {\dataDir/laplace_penalty_non_matching_proj_SIMPLE_SIMPLE_condest_p2.txt};
    \addlegendentry{$p=2$, SIMPLE};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 5] {\dataDir/laplace_penalty_non_matching_proj_SIMPLE_SIMPLE_condest_p3.txt};
    \addlegendentry{$p=3$, SIMPLE};

    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 5] {\dataDir/laplace_penalty_non_matching_proj_SIMPLE_SIMPLE_condest_p4.txt};
    \addlegendentry{$p=4$, SIMPLE};


%\logLogSlopeReverseTriangle{0.85}{0.08}{0.445}{2}{black};
%\logLogSlopeReverseTriangle{0.85}{0.08}{0.25}{3}{black};
%\logLogSlopeReverseTriangle{0.85}{0.08}{0.0625}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};

\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_laplace_curved_nonconforming_ilu.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^1$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west,
skip coords between index={7}{8}
]


	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{3}^0.5, y index = 1] {\dataDir/laplace_penalty_non_matching_no_proj_SIMPLE_ILU_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 1] {\dataDir/laplace_penalty_non_matching_no_proj_SIMPLE_ILU_p3.txt};
    \addlegendentry{$p=3$};

    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 1] {\dataDir/laplace_penalty_non_matching_no_proj_SIMPLE_ILU_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{3}^0.5, y index = 1] {\dataDir/laplace_penalty_non_matching_proj_SIMPLE_ILU_p2.txt};
    \addlegendentry{$p=2, p^{red}=0$};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 1] {\dataDir/laplace_penalty_non_matching_proj_SIMPLE_ILU_p3.txt};
    \addlegendentry{$p=3, p^{red}=1$};

    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 1] {\dataDir/laplace_penalty_non_matching_proj_SIMPLE_ILU_p4.txt};
    \addlegendentry{$p=4, p^{red}=2$};


%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.445}{2}{black};
\logLogSlopeReverseTriangle{0.85}{0.08}{0.25}{3}{black};
\logLogSlopeReverseTriangle{0.85}{0.08}{0.0625}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_laplace_curved_nonconforming_no_precond_condest.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Condition number,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= north west,
%skip coords between index={7}{8}
]

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{3}^0.5, y index = 5] {\dataDir/laplace_penalty_non_matching_proj_NO_PRECOND_condest_p2.txt};
    \addlegendentry{$p=2, p^{red}=0$};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 5] {\dataDir/laplace_penalty_non_matching_proj_NO_PRECOND_condest_p3.txt};
    \addlegendentry{$p=3, p^{red}=1$};

    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 5] {\dataDir/laplace_penalty_non_matching_proj_NO_PRECOND_condest_p4.txt};
    \addlegendentry{$p=4, p^{red}=2$};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};



\logLogSlopeTriangle{0.9}{0.08}{0.47}{3}{black};
\logLogSlopeTriangle{0.9}{0.08}{0.64}{4}{black};
\logLogSlopeTriangle{0.9}{0.08}{0.82}{5}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};

\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_laplace_nonconforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^1$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/laplace_coupling_2patches_nonconforming_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/laplace_coupling_2patches_nonconforming_p3.txt};
    \addlegendentry{$p=3$};


%    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/laplace_coupling_2patches_nonconforming_p4.txt};
%    \addlegendentry{$p=4$};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/laplace_coupling_2patches_nonconforming_projected_p2.txt};
    \addlegendentry{$p=2, p^{red}=0$};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/laplace_coupling_2patches_nonconforming_projected_p3.txt};
    \addlegendentry{$p=3, p^{red}=1$};

%    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/laplace_coupling_2patches_nonconforming_projected_p4.txt};
%    \addlegendentry{$p=4, p^{red}=2$};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.335}{2}{black};
\logLogSlopeReverseTriangle{0.82}{0.08}{0.0625}{3}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_laplace_trimmed_conforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^1$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/laplace_trimmed_coupling_2patches_conforming_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/laplace_trimmed_coupling_2patches_conforming_p3.txt};
    \addlegendentry{$p=3$};


    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/laplace_trimmed_coupling_2patches_conforming_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/laplace_trimmed_coupling_2patches_conforming_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/laplace_trimmed_coupling_2patches_conforming_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/laplace_trimmed_coupling_2patches_conforming_projected_p4.txt};
    \addlegendentry{$p=4$ proj};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.52}{2}{black};
\logLogSlopeReverseTriangle{0.85}{0.08}{0.245}{3}{black};
\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_scordelislo_curved_conforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
xmax=2.5e2,
xminorticks=true,
%ymode=log,
ymin=0.01,
ymax=1.2,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Normalized displacement,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south east
]
	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y expr=\thisrowno{1}/(-0.3005925)] {\dataDir/shell_scordelislo_coupling_2patches_conforming_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y expr=\thisrowno{1}/(-0.3005925)] {\dataDir/shell_scordelislo_coupling_2patches_conforming_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y expr=\thisrowno{1}/(-0.3005925)] {\dataDir/shell_scordelislo_coupling_2patches_conforming_breitenberger_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y expr=\thisrowno{1}/(-0.3005925)] {\dataDir/shell_scordelislo_coupling_2patches_conforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y expr=\thisrowno{1}/(-0.3005925)] {\dataDir/shell_scordelislo_coupling_2patches_conforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y expr=\thisrowno{1}/(-0.3005925)] {\dataDir/shell_scordelislo_coupling_2patches_conforming_p4.txt};
    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y expr=\thisrowno{1}/(-0.3005925)] {\dataDir/shell_scordelislo_coupling_2patches_conforming_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y expr=\thisrowno{1}/(-0.3005925)] {\dataDir/shell_scordelislo_coupling_2patches_conforming_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y expr=\thisrowno{1}/(-0.3005925)] {\dataDir/shell_scordelislo_coupling_2patches_conforming_projected_p4.txt};
    \addlegendentry{$p=4$ proj};

%    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_tilted_coupling_2patches_conforming_projected_p4.txt};
%    \addlegendentry{$p=4, p^{red}=2$};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
%\logLogSlopeReverseTriangle{0.85}{0.08}{0.62}{1}{black};
%\logLogSlopeReverseTriangle{0.82}{0.08}{0.33}{2}{black};
%\logLogSlopeReverseTriangle{0.82}{0.08}{0.06}{3}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_scordelislo_curved_fineMaster_nonconforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
xmax=1.5e2,
xminorticks=true,
%ymode=log,
ymin=0.01,
ymax=1.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Normalized displacement,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= outer north east,
]
	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y expr=\thisrowno{1}/(-0.3005925)] {\dataDir/shell_scordelislo_coupling_2patches_nonconforming_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y expr=\thisrowno{1}/(-0.3005925)] {\dataDir/shell_scordelislo_coupling_2patches_nonconforming_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y expr=\thisrowno{1}/(-0.3005925)] {\dataDir/shell_scordelislo_coupling_2patches_nonconforming_breitenberger_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y expr=\thisrowno{1}/(-0.3005925)] {\dataDir/shell_scordelislo_coupling_2patches_nonconforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y expr=\thisrowno{1}/(-0.3005925)] {\dataDir/shell_scordelislo_coupling_2patches_nonconforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y expr=\thisrowno{1}/(-0.3005925)] {\dataDir/shell_scordelislo_coupling_2patches_nonconforming_p4.txt};
    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y expr=\thisrowno{1}/(-0.3005925)] {\dataDir/shell_scordelislo_coupling_fineMaster_2patches_nonconforming_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y expr=\thisrowno{1}/(-0.3005925)] {\dataDir/shell_scordelislo_coupling_fineMaster_2patches_nonconforming_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y expr=\thisrowno{1}/(-0.3005925)] {\dataDir/shell_scordelislo_coupling_fineMaster_2patches_nonconforming_projected_p4.txt};
    \addlegendentry{$p=4$ proj};


\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_scordelislo_curved_nonconforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
xmax=2.5e2,
xminorticks=true,
%ymode=log,
ymin=0.01,
ymax=1.2,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Normalized displacement,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south east
]
	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y expr=\thisrowno{1}/(-0.3005925)] {\dataDir/shell_scordelislo_coupling_2patches_nonconforming_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y expr=\thisrowno{1}/(-0.3005925)] {\dataDir/shell_scordelislo_coupling_2patches_nonconforming_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y expr=\thisrowno{1}/(-0.3005925)] {\dataDir/shell_scordelislo_coupling_2patches_nonconforming_breitenberger_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y expr=\thisrowno{1}/(-0.3005925)] {\dataDir/shell_scordelislo_coupling_2patches_nonconforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y expr=\thisrowno{1}/(-0.3005925)] {\dataDir/shell_scordelislo_coupling_2patches_nonconforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y expr=\thisrowno{1}/(-0.3005925)] {\dataDir/shell_scordelislo_coupling_2patches_nonconforming_p4.txt};
    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y expr=\thisrowno{1}/(-0.3005925)] {\dataDir/shell_scordelislo_coupling_2patches_nonconforming_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y expr=\thisrowno{1}/(-0.3005925)] {\dataDir/shell_scordelislo_coupling_2patches_nonconforming_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y expr=\thisrowno{1}/(-0.3005925)] {\dataDir/shell_scordelislo_coupling_2patches_nonconforming_projected_p4.txt};
    \addlegendentry{$p=4$ proj};

%    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_tilted_coupling_2patches_conforming_projected_p4.txt};
%    \addlegendentry{$p=4, p^{red}=2$};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
%\logLogSlopeReverseTriangle{0.85}{0.08}{0.62}{1}{black};
%\logLogSlopeReverseTriangle{0.82}{0.08}{0.33}{2}{black};
%\logLogSlopeReverseTriangle{0.82}{0.08}{0.06}{3}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_scordelislo_trimmed_curved_conforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
xmax=1.2e2,
xminorticks=true,
%ymode=log,
ymin=0.01,
ymax=1.2,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Normalized displacement,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south east,
skip coords between index={0}{1}
]
	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{1}^0.5, y expr=\thisrowno{0}/(-0.3005925)] {\dataDir/shell_scordelislo_trimmed_coupling_2patches_conforming_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{1}^0.5, y expr=\thisrowno{0}/(-0.3005925)] {\dataDir/shell_scordelislo_trimmed_coupling_2patches_conforming_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{1}^0.5, y expr=\thisrowno{0}/(-0.3005925)] {\dataDir/shell_scordelislo_trimmed_coupling_2patches_conforming_breitenberger_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{1}^0.5, y expr=\thisrowno{0}/(-0.3005925)] {\dataDir/shell_scordelislo_trimmed_coupling_2patches_conforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{1}^0.5, y expr=\thisrowno{0}/(-0.3005925)] {\dataDir/shell_scordelislo_trimmed_coupling_2patches_conforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{1}^0.5, y expr=\thisrowno{0}/(-0.3005925)] {\dataDir/shell_scordelislo_trimmed_coupling_2patches_conforming_p4.txt};
    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{1}^0.5, y expr=\thisrowno{0}/(-0.3005925)] {\dataDir/shell_scordelislo_trimmed_coupling_2patches_conforming_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{1}^0.5, y expr=\thisrowno{0}/(-0.3005925)] {\dataDir/shell_scordelislo_trimmed_coupling_2patches_conforming_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{1}^0.5, y expr=\thisrowno{0}/(-0.3005925)] {\dataDir/shell_scordelislo_trimmed_coupling_2patches_conforming_projected_p4.txt};
    \addlegendentry{$p=4$ proj};


\end{axis}
\end{tikzpicture}%




==> pictures/numericalExamples/graphs/convergence_scordelislo_trimmed_curved_fineMaster_nonconforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
xmax=1.2e2,
xminorticks=true,
%ymode=log,
ymin=0.01,
ymax=1.2,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Normalized displacement,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south east,
skip coords between index={0}{1}
]
	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{1}^0.5, y expr=\thisrowno{0}/(-0.3005925)] {\dataDir/shell_scordelislo_trimmed_coupling_2patches_nonConforming_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{1}^0.5, y expr=\thisrowno{0}/(-0.3005925)] {\dataDir/shell_scordelislo_trimmed_coupling_2patches_nonConforming_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{1}^0.5, y expr=\thisrowno{0}/(-0.3005925)] {\dataDir/shell_scordelislo_trimmed_coupling_2patches_nonConforming_breitenberger_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{1}^0.5, y expr=\thisrowno{0}/(-0.3005925)] {\dataDir/shell_scordelislo_trimmed_coupling_2patches_nonConforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{1}^0.5, y expr=\thisrowno{0}/(-0.3005925)] {\dataDir/shell_scordelislo_trimmed_coupling_2patches_nonConforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{1}^0.5, y expr=\thisrowno{0}/(-0.3005925)] {\dataDir/shell_scordelislo_trimmed_coupling_2patches_nonConforming_p4.txt};
    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{1}^0.5, y expr=\thisrowno{0}/(-0.3005925)] {\dataDir/shell_scordelislo_trimmed_coupling_2patches_nonConforming_fineMaster_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{1}^0.5, y expr=\thisrowno{0}/(-0.3005925)] {\dataDir/shell_scordelislo_trimmed_coupling_2patches_nonConforming_fineMaster_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{1}^0.5, y expr=\thisrowno{0}/(-0.3005925)] {\dataDir/shell_scordelislo_trimmed_coupling_2patches_nonConforming_fineMaster_projected_p4.txt};
    \addlegendentry{$p=4$ proj};


\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_scordelislo_trimmed_curved_nonconforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
xmax=1.2e2,
xminorticks=true,
%ymode=log,
ymin=0.01,
ymax=1.2,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Normalized displacement,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south east,
skip coords between index={0}{1}
]
	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{1}^0.5, y expr=\thisrowno{0}/(-0.3005925)] {\dataDir/shell_scordelislo_trimmed_coupling_2patches_nonConforming_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{1}^0.5, y expr=\thisrowno{0}/(-0.3005925)] {\dataDir/shell_scordelislo_trimmed_coupling_2patches_nonConforming_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{1}^0.5, y expr=\thisrowno{0}/(-0.3005925)] {\dataDir/shell_scordelislo_trimmed_coupling_2patches_nonConforming_breitenberger_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{1}^0.5, y expr=\thisrowno{0}/(-0.3005925)] {\dataDir/shell_scordelislo_trimmed_coupling_2patches_nonConforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{1}^0.5, y expr=\thisrowno{0}/(-0.3005925)] {\dataDir/shell_scordelislo_trimmed_coupling_2patches_nonConforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{1}^0.5, y expr=\thisrowno{0}/(-0.3005925)] {\dataDir/shell_scordelislo_trimmed_coupling_2patches_nonConforming_p4.txt};
    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{1}^0.5, y expr=\thisrowno{0}/(-0.3005925)] {\dataDir/shell_scordelislo_trimmed_coupling_2patches_nonConforming_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{1}^0.5, y expr=\thisrowno{0}/(-0.3005925)] {\dataDir/shell_scordelislo_trimmed_coupling_2patches_nonConforming_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{1}^0.5, y expr=\thisrowno{0}/(-0.3005925)] {\dataDir/shell_scordelislo_trimmed_coupling_2patches_nonConforming_projected_p4.txt};
    \addlegendentry{$p=4$ proj};


\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_shell_curved_conforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^2$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west
]
	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_curved_coupling_2patches_conforming_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_curved_coupling_2patches_conforming_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_curved_coupling_2patches_conforming_breitenberger_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_curved_coupling_2patches_conforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_curved_coupling_2patches_conforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_curved_coupling_2patches_conforming_p4.txt};
    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_curved_coupling_2patches_conforming_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_curved_coupling_2patches_conforming_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_curved_coupling_2patches_conforming_projected_p4.txt};
    \addlegendentry{$p=4$ proj};

%    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_tilted_coupling_2patches_conforming_projected_p4.txt};
%    \addlegendentry{$p=4, p^{red}=2$};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.62}{1}{black};
\logLogSlopeReverseTriangle{0.82}{0.08}{0.33}{2}{black};
\logLogSlopeReverseTriangle{0.82}{0.08}{0.06}{3}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_shell_curved_cut_trimmed_conforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1.5e2,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^2$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west,
skip coords between index={0}{1}
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/shell_trimmed_curved_cut_2patches_fromFile_breitenberger_conforming_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/shell_trimmed_curved_cut_2patches_fromFile_breitenberger_conforming_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/shell_trimmed_curved_cut_2patches_fromFile_breitenberger_conforming_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/shell_trimmed_curved_cut_2patches_fromFile_conforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/shell_trimmed_curved_cut_2patches_fromFile_conforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/shell_trimmed_curved_cut_2patches_fromFile_conforming_p4.txt};
    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/shell_trimmed_curved_cut_coupling_2patches_projected_conforming_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/shell_trimmed_curved_cut_coupling_2patches_projected_conforming_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/shell_trimmed_curved_cut_coupling_2patches_projected_conforming_p4.txt};
    \addlegendentry{$p=4$ proj};

{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.625}{1}{black};
\logLogSlopeReverseTriangle{0.85}{0.08}{0.27}{2}{black};
\logLogSlopeReverseTriangle{0.82}{0.08}{0.055}{3}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_shell_curved_cut_trimmed_nonconforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
xmax=1.e2,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^2$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west,
skip coords between index={5}{6}
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/shell_trimmed_curved_cut_2patches_breitenberger_nonConforming_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/shell_trimmed_curved_cut_2patches_breitenberger_nonConforming_p3.txt};
    \addlegendentry{$p=3$};

%	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/shell_trimmed_curved_cut_2patches_breitenberger_nonConforming_p4.txt};
%    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/shell_trimmed_curved_cut_2patches_nonConforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/shell_trimmed_curved_cut_2patches_nonConforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

%	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/shell_trimmed_curved_cut_2patches_nonConforming_p4.txt};
%    \addlegendentry{$p=4$ scaled};

%	\addplot [color=c1, dashed,mark=o,mark options={solid}]
%    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/shell_trimmed_curved_cut_coupling_2patches_projected_fineMaster_nonConforming_p2.txt};
%    \addlegendentry{$p=2$ proj};
%	
%	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/shell_trimmed_curved_cut_coupling_2patches_projected_fineMaster_nonConforming_p3.txt};
%    \addlegendentry{$p=3$ proj};
%
%	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/shell_trimmed_curved_cut_coupling_2patches_projected_fineMaster_nonConforming_p4.txt};
    \addlegendentry{$p=4$ proj};
	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/shell_trimmed_curved_cut_coupling_2patches_projected_nonConforming_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/shell_trimmed_curved_cut_coupling_2patches_projected_nonConforming_p3.txt};
    \addlegendentry{$p=3$ proj};

%	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 2] {\dataDir/shell_trimmed_curved_cut_coupling_2patches_projected_nonConforming_p4.txt};
%    \addlegendentry{$p=4$ proj};

{
\logLogSlopeReverseTriangle{0.78}{0.08}{0.545}{1}{black};
\logLogSlopeReverseTriangle{0.735}{0.08}{0.055}{2}{black};
%\logLogSlopeReverseTriangle{0.85}{0.08}{0.055}{3}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_shell_curved_cut_trimmed_nonconforming_h1.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
xmax=1.e2,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^1$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west,
skip coords between index={5}{6}
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/shell_trimmed_curved_cut_2patches_breitenberger_nonConforming_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/shell_trimmed_curved_cut_2patches_breitenberger_nonConforming_p3.txt};
    \addlegendentry{$p=3$};

%	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/shell_trimmed_curved_cut_2patches_breitenberger_nonConforming_p4.txt};
%    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/shell_trimmed_curved_cut_2patches_nonConforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/shell_trimmed_curved_cut_2patches_nonConforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

%	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/shell_trimmed_curved_cut_2patches_nonConforming_p4.txt};
%    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/shell_trimmed_curved_cut_coupling_2patches_projected_nonConforming_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/shell_trimmed_curved_cut_coupling_2patches_projected_nonConforming_p3.txt};
    \addlegendentry{$p=3$ proj};

%	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/shell_trimmed_curved_cut_coupling_2patches_projected_nonConforming_p4.txt};
%    \addlegendentry{$p=4$ proj};



{
\logLogSlopeReverseTriangle{0.78}{0.08}{0.365}{2}{black};
\logLogSlopeReverseTriangle{0.73}{0.08}{0.055}{3}{black};
%\logLogSlopeReverseTriangle{0.82}{0.08}{0.055}{4}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_shell_curved_cut_trimmed_nonconforming_l2.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
xmax=1.e2,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $L^2$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west,
skip coords between index={5}{6}
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 0] {\dataDir/shell_trimmed_curved_cut_2patches_breitenberger_nonConforming_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 0] {\dataDir/shell_trimmed_curved_cut_2patches_breitenberger_nonConforming_p3.txt};
    \addlegendentry{$p=3$};

%	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 0] {\dataDir/shell_trimmed_curved_cut_2patches_breitenberger_nonConforming_p4.txt};
%    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 0] {\dataDir/shell_trimmed_curved_cut_2patches_nonConforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 0] {\dataDir/shell_trimmed_curved_cut_2patches_nonConforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

%	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 0] {\dataDir/shell_trimmed_curved_cut_2patches_nonConforming_p4.txt};
%    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 0] {\dataDir/shell_trimmed_curved_cut_coupling_2patches_projected_nonConforming_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 0] {\dataDir/shell_trimmed_curved_cut_coupling_2patches_projected_nonConforming_p3.txt};
    \addlegendentry{$p=3$ proj};

%	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 0] {\dataDir/shell_trimmed_curved_cut_coupling_2patches_projected_nonConforming_p4.txt};
%    \addlegendentry{$p=4$ proj};

{
\logLogSlopeReverseTriangle{0.78}{0.08}{0.415}{2}{black};
\logLogSlopeReverseTriangle{0.735}{0.08}{0.055}{4}{black};
%\logLogSlopeReverseTriangle{0.64}{0.08}{0.055}{5}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_shell_curved_nonconforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^2$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west
]


	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_curved_coupling_2patches_nonconforming_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_curved_coupling_2patches_nonconforming_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_curved_coupling_2patches_nonconforming_breitenberger_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_curved_coupling_2patches_nonconforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_curved_coupling_2patches_nonconforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_curved_coupling_2patches_nonconforming_p4.txt};
    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_curved_coupling_2patches_nonconforming_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_curved_coupling_2patches_nonconforming_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_curved_coupling_2patches_nonconforming_projected_p4.txt};
    \addlegendentry{$p=4$ proj};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.615}{1}{black};
\logLogSlopeReverseTriangle{0.8}{0.08}{0.35}{2}{black};
\logLogSlopeReverseTriangle{0.8}{0.08}{0.08}{3}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_shell_curved_nonconforming_h1.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^1$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west
]


	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/shell_curved_coupling_2patches_nonconforming_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/shell_curved_coupling_2patches_nonconforming_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/shell_curved_coupling_2patches_nonconforming_breitenberger_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/shell_curved_coupling_2patches_nonconforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/shell_curved_coupling_2patches_nonconforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/shell_curved_coupling_2patches_nonconforming_p4.txt};
    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/shell_curved_coupling_2patches_nonconforming_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/shell_curved_coupling_2patches_nonconforming_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/shell_curved_coupling_2patches_nonconforming_projected_p4.txt};
    \addlegendentry{$p=4$ proj};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.465}{2}{black};
\logLogSlopeReverseTriangle{0.85}{0.08}{0.255}{3}{black};
\logLogSlopeReverseTriangle{0.8}{0.08}{0.08}{4}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_shell_curved_nonconforming_l2.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $L^2$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west
]


	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_curved_coupling_2patches_nonconforming_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_curved_coupling_2patches_nonconforming_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_curved_coupling_2patches_nonconforming_breitenberger_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_curved_coupling_2patches_nonconforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_curved_coupling_2patches_nonconforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_curved_coupling_2patches_nonconforming_p4.txt};
    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_curved_coupling_2patches_nonconforming_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_curved_coupling_2patches_nonconforming_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_curved_coupling_2patches_nonconforming_projected_p4.txt};
    \addlegendentry{$p=4$ proj};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.445}{2}{black};
\logLogSlopeReverseTriangle{0.85}{0.08}{0.24}{4}{black};
\logLogSlopeReverseTriangle{0.8}{0.08}{0.08}{5}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_shell_diagonal_trimmed_conforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1.5e2,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^2$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_coupling_trimmed_diagonal_conforming_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_coupling_trimmed_diagonal_conforming_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_coupling_trimmed_diagonal_conforming_breitenberger_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_coupling_trimmed_diagonal_conforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_coupling_trimmed_diagonal_conforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_coupling_trimmed_diagonal_conforming_p4.txt};
    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_coupling_trimmed_diagonal_conforming_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_coupling_trimmed_diagonal_conforming_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_coupling_trimmed_diagonal_conforming_projected_p4.txt};
    \addlegendentry{$p=4$ proj};

{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.655}{1}{black};
\logLogSlopeReverseTriangle{0.85}{0.08}{0.32}{2}{black};
\logLogSlopeReverseTriangle{0.85}{0.08}{0.055}{3}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_shell_diagonal_trimmed_nonconforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1.5e2,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^2$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_coupling_trimmed_diagonal_nonConforming_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_coupling_trimmed_diagonal_nonConforming_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_coupling_trimmed_diagonal_nonConforming_breitenberger_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_coupling_trimmed_diagonal_nonConforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_coupling_trimmed_diagonal_nonConforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_coupling_trimmed_diagonal_nonConforming_p4.txt};
    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_coupling_trimmed_diagonal_nonConforming_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_coupling_trimmed_diagonal_nonConforming_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_coupling_trimmed_diagonal_nonConforming_projected_p4.txt};
    \addlegendentry{$p=4$ proj};

{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.675}{1}{black};
\logLogSlopeReverseTriangle{0.85}{0.08}{0.35}{2}{black};
\logLogSlopeReverseTriangle{0.85}{0.08}{0.055}{3}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_shell_diagonal_trimmed_nonconforming_h1.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1.5e2,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^1$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/shell_coupling_trimmed_diagonal_nonConforming_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/shell_coupling_trimmed_diagonal_nonConforming_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/shell_coupling_trimmed_diagonal_nonConforming_breitenberger_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/shell_coupling_trimmed_diagonal_nonConforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/shell_coupling_trimmed_diagonal_nonConforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/shell_coupling_trimmed_diagonal_nonConforming_p4.txt};
    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/shell_coupling_trimmed_diagonal_nonConforming_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/shell_coupling_trimmed_diagonal_nonConforming_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/shell_coupling_trimmed_diagonal_nonConforming_projected_p4.txt};
    \addlegendentry{$p=4$ proj};



{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.515}{2}{black};
\logLogSlopeReverseTriangle{0.85}{0.08}{0.235}{3}{black};
\logLogSlopeReverseTriangle{0.82}{0.08}{0.055}{4}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_shell_diagonal_trimmed_nonconforming_l2.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1.5e2,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $L^2$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_coupling_trimmed_diagonal_nonConforming_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_coupling_trimmed_diagonal_nonConforming_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_coupling_trimmed_diagonal_nonConforming_breitenberger_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_coupling_trimmed_diagonal_nonConforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_coupling_trimmed_diagonal_nonConforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_coupling_trimmed_diagonal_nonConforming_p4.txt};
    \addlegendentry{$p=4$ scaled};

%    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_tilted_coupling_2patches_conforming_p4.txt};
%    \addlegendentry{$p=4$};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_coupling_trimmed_diagonal_nonConforming_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_coupling_trimmed_diagonal_nonConforming_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_coupling_trimmed_diagonal_nonConforming_projected_p4.txt};
    \addlegendentry{$p=4$ proj};

%    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_tilted_coupling_2patches_conforming_projected_p4.txt};
%    \addlegendentry{$p=4, p^{red}=2$};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.485}{2}{black};
\logLogSlopeReverseTriangle{0.85}{0.08}{0.18}{4}{black};
\logLogSlopeReverseTriangle{0.64}{0.08}{0.055}{5}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_shell_trimmed_conforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^2$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_trimmed_coupling_2patches_fromFile_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_trimmed_coupling_2patches_fromFile_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_trimmed_coupling_2patches_fromFile_breitenberger_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_trimmed_coupling_2patches_fromFile_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_trimmed_coupling_2patches_fromFile_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_trimmed_coupling_2patches_fromFile_p4.txt};
    \addlegendentry{$p=4$ scaled};

%    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_tilted_coupling_2patches_conforming_p4.txt};
%    \addlegendentry{$p=4$};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_trimmed_coupling_2patches_fromFile_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_trimmed_coupling_2patches_fromFile_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_trimmed_coupling_2patches_fromFile_projected_p4.txt};
    \addlegendentry{$p=4$ proj};

%    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_tilted_coupling_2patches_conforming_projected_p4.txt};
%    \addlegendentry{$p=4, p^{red}=2$};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.65}{1}{black};
\logLogSlopeReverseTriangle{0.85}{0.08}{0.31}{2}{black};
\logLogSlopeReverseTriangle{0.835}{0.08}{0.055}{3}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_shell_trimmed_conforming_h1.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^1$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/shell_trimmed_coupling_2patches_fromFile_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/shell_trimmed_coupling_2patches_fromFile_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/shell_trimmed_coupling_2patches_fromFile_breitenberger_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/shell_trimmed_coupling_2patches_fromFile_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/shell_trimmed_coupling_2patches_fromFile_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/shell_trimmed_coupling_2patches_fromFile_p4.txt};
    \addlegendentry{$p=4$ scaled};

%    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_tilted_coupling_2patches_conforming_p4.txt};
%    \addlegendentry{$p=4$};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/shell_trimmed_coupling_2patches_fromFile_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/shell_trimmed_coupling_2patches_fromFile_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/shell_trimmed_coupling_2patches_fromFile_projected_p4.txt};
    \addlegendentry{$p=4$ proj};

%    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_tilted_coupling_2patches_conforming_projected_p4.txt};
%    \addlegendentry{$p=4, p^{red}=2$};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.465}{2}{black};
\logLogSlopeReverseTriangle{0.85}{0.08}{0.22}{3}{black};
\logLogSlopeReverseTriangle{0.825}{0.08}{0.055}{4}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_shell_trimmed_conforming_l2.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $L^2$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_trimmed_coupling_2patches_fromFile_breitenberger_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_trimmed_coupling_2patches_fromFile_breitenberger_p3.txt};
    \addlegendentry{$p=3$};

	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_trimmed_coupling_2patches_fromFile_breitenberger_p4.txt};
    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_trimmed_coupling_2patches_fromFile_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_trimmed_coupling_2patches_fromFile_p3.txt};
    \addlegendentry{$p=3$ scaled};

	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_trimmed_coupling_2patches_fromFile_p4.txt};
    \addlegendentry{$p=4$ scaled};

%    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_tilted_coupling_2patches_conforming_p4.txt};
%    \addlegendentry{$p=4$};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_trimmed_coupling_2patches_fromFile_projected_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_trimmed_coupling_2patches_fromFile_projected_p3.txt};
    \addlegendentry{$p=3$ proj};

	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_trimmed_coupling_2patches_fromFile_projected_p4.txt};
    \addlegendentry{$p=4$ proj};

%    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/bilaplace_tilted_coupling_2patches_conforming_projected_p4.txt};
%    \addlegendentry{$p=4, p^{red}=2$};

%    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
%    \addlegendentry{$p=5$};
%
%    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
%    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
%    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.405}{2}{black};
\logLogSlopeReverseTriangle{0.85}{0.08}{0.155}{4}{black};
\logLogSlopeReverseTriangle{0.66}{0.08}{0.065}{5}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_shell_trimmed_nonconforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^2$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_trimmed_coupling_2patches_fromFile_breitenberger_nonConforming_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_trimmed_coupling_2patches_fromFile_breitenberger_nonConforming_p3.txt};
    \addlegendentry{$p=3$};

%	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_trimmed_coupling_2patches_fromFile_breitenberger_nonConforming_p4.txt};
%    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_trimmed_coupling_2patches_fromFile_nonConforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_trimmed_coupling_2patches_fromFile_nonConforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

%	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_trimmed_coupling_2patches_fromFile_nonConforming_p4.txt};
%    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_trimmed_coupling_2patches_fromFile_projected_nonConforming_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_trimmed_coupling_2patches_fromFile_projected_nonConforming_p3.txt};
    \addlegendentry{$p=3$ proj};

%	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{5}^0.5, y index = 3] {\dataDir/shell_trimmed_coupling_2patches_fromFile_projected_nonConforming_p4.txt};
%    \addlegendentry{$p=4$ proj};

{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.555}{1}{black};
\logLogSlopeReverseTriangle{0.85}{0.08}{0.055}{2}{black};
%\logLogSlopeReverseTriangle{0.45}{0.08}{0.17}{3}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_shell_trimmed_nonconforming_h1.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^1$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/shell_trimmed_coupling_2patches_fromFile_breitenberger_nonConforming_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/shell_trimmed_coupling_2patches_fromFile_breitenberger_nonConforming_p3.txt};
    \addlegendentry{$p=3$};

%	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/shell_trimmed_coupling_2patches_fromFile_breitenberger_nonConforming_p4.txt};
%    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/shell_trimmed_coupling_2patches_fromFile_nonConforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/shell_trimmed_coupling_2patches_fromFile_nonConforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

%	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/shell_trimmed_coupling_2patches_fromFile_nonConforming_p4.txt};
%    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/shell_trimmed_coupling_2patches_fromFile_projected_nonConforming_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 2] {\dataDir/shell_trimmed_coupling_2patches_fromFile_projected_nonConforming_p3.txt};
    \addlegendentry{$p=3$ proj};

%	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 1] {\dataDir/shell_trimmed_coupling_2patches_fromFile_projected_nonConforming_p4.txt};
%    \addlegendentry{$p=4$ proj};
    

{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.335}{2}{black};
\logLogSlopeReverseTriangle{0.82}{0.08}{0.055}{3}{black};
%\logLogSlopeReverseTriangle{0.625}{0.08}{0.085}{4}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_shell_trimmed_nonconforming_l2.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $L^2$ norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_trimmed_coupling_2patches_fromFile_breitenberger_nonConforming_p2.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_trimmed_coupling_2patches_fromFile_breitenberger_nonConforming_p3.txt};
    \addlegendentry{$p=3$};

%	\addplot[color=c3, solid, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 0] {\dataDir/shell_trimmed_curved_cut_2patches_fromFile_breitenberger_nonConforming_p4.txt};
%    \addlegendentry{$p=4$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_trimmed_coupling_2patches_fromFile_nonConforming_p2.txt};
    \addlegendentry{$p=2$ scaled};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_trimmed_coupling_2patches_fromFile_nonConforming_p3.txt};
    \addlegendentry{$p=3$ scaled};

%	\addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 0] {\dataDir/shell_trimmed_coupling_2patches_fromFile_nonConforming_p4.txt};
%    \addlegendentry{$p=4$ scaled};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_trimmed_coupling_2patches_fromFile_projected_nonConforming_p2.txt};
    \addlegendentry{$p=2$ proj};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{5}^0.5, y index = 1] {\dataDir/shell_trimmed_coupling_2patches_fromFile_projected_nonConforming_p3.txt};
    \addlegendentry{$p=3$ proj};

%	\addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
%    table[ x expr=\thisrowno{4}^0.5, y index = 0] {\dataDir/shell_trimmed_coupling_2patches_fromFile_projected_nonConforming_p4.txt};
%    \addlegendentry{$p=4$ proj};

{
\logLogSlopeReverseTriangle{0.85}{0.08}{0.3051}{2}{black};
\logLogSlopeReverseTriangle{0.82}{0.08}{0.055}{4}{black};
%\logLogSlopeReverseTriangle{0.61}{0.08}{0.055}{5}{black};
%\logLogSlopeReverseTriangle{0.8175}{0.08}{0.07}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_weak_penalty_condition_beta1e12.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Condition number,
%xlabel= Mesh size $h$,
xlabel= mesh size $h$,
legend style={font=\tiny},
legend pos= south west
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x index = 0, y index = 4] {\dataDir/plate_weak_dirichlet_p2_beta1e12.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x index = 0, y index = 4] {\dataDir/plate_weak_dirichlet_p3_beta1e12.txt};
    \addlegendentry{$p=3$};

    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x index = 0, y index = 4] {\dataDir/plate_weak_dirichlet_p4_beta1e12.txt};
    \addlegendentry{$p=4$};

    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
    table[ x index = 0, y index = 4] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
    \addlegendentry{$p=5$};

    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
    table[ x index = 0, y index = 4] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
%\logLogSlopeTriangle{0.39}{0.08}{0.15}{3}{black};
%\logLogSlopeTriangle{0.55}{0.08}{0.325}{1}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.095}{5}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.095}{6}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.095}{7}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_weak_penalty_condition_beta1e3.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Condition number,
%xlabel= Mesh size $h$,
xlabel= mesh size $h$,
legend style={font=\tiny},
legend pos= south west
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x index = 0, y index = 4] {\dataDir/plate_weak_dirichlet_p2_beta1e3.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x index = 0, y index = 4] {\dataDir/plate_weak_dirichlet_p3_beta1e3.txt};
    \addlegendentry{$p=3$};

    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x index = 0, y index = 4] {\dataDir/plate_weak_dirichlet_p4_beta1e3.txt};
    \addlegendentry{$p=4$};

    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
    table[ x index = 0, y index = 4] {\dataDir/plate_weak_dirichlet_p5_beta1e3.txt};
    \addlegendentry{$p=5$};

    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
    table[ x index = 0, y index = 4] {\dataDir/plate_weak_dirichlet_p6_beta1e3.txt};
    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
%\logLogSlopeTriangle{0.39}{0.08}{0.15}{3}{black};
%\logLogSlopeTriangle{0.55}{0.08}{0.325}{1}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.095}{5}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.095}{6}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.095}{7}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_weak_penalty_condition_beta1e6.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Condition number,
%xlabel= Mesh size $h$,
xlabel= mesh size $h$,
legend style={font=\tiny},
legend pos= south west
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x index = 0, y index = 4] {\dataDir/plate_weak_dirichlet_p2_beta1e6.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x index = 0, y index = 4] {\dataDir/plate_weak_dirichlet_p3_beta1e6.txt};
    \addlegendentry{$p=3$};

    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x index = 0, y index = 4] {\dataDir/plate_weak_dirichlet_p4_beta1e6.txt};
    \addlegendentry{$p=4$};

    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
    table[ x index = 0, y index = 4] {\dataDir/plate_weak_dirichlet_p5_beta1e6.txt};
    \addlegendentry{$p=5$};

    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
    table[ x index = 0, y index = 4] {\dataDir/plate_weak_dirichlet_p6_beta1e6.txt};
    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
%\logLogSlopeTriangle{0.39}{0.08}{0.15}{3}{black};
%\logLogSlopeTriangle{0.55}{0.08}{0.325}{1}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.095}{5}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.095}{6}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.095}{7}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_weak_penalty_h1_beta1e12.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^1$ semi-norm,
%xlabel= Mesh size $h$,
xlabel= mesh size $h$,
legend style={font=\tiny},
legend pos= south east
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x index = 0, y index = 2] {\dataDir/plate_weak_dirichlet_p2_beta1e12.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x index = 0, y index = 2] {\dataDir/plate_weak_dirichlet_p3_beta1e12.txt};
    \addlegendentry{$p=3$};


    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x index = 0, y index = 2] {\dataDir/plate_weak_dirichlet_p4_beta1e12.txt};
    \addlegendentry{$p=4$};

    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
    table[ x index = 0, y index = 2] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
    \addlegendentry{$p=5$};

    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
    table[ x index = 0, y index = 2] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
\logLogSlopeTriangle{0.19}{0.08}{0.65}{2}{black};
\logLogSlopeTriangle{0.19}{0.08}{0.46}{3}{black};
\logLogSlopeTriangle{0.19}{0.08}{0.28}{4}{black};
\logLogSlopeTriangle{0.19}{0.08}{0.12}{5}{black};
\logLogSlopeTriangle{0.36}{0.08}{0.09}{6}{black};

}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_weak_penalty_h1_beta1e3.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^1$ semi-norm,
%xlabel= Mesh size $h$,
xlabel= mesh size $h$,
legend style={font=\tiny},
legend pos= south east
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x index = 0, y index = 2] {\dataDir/plate_weak_dirichlet_p2_beta1e3.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x index = 0, y index = 2] {\dataDir/plate_weak_dirichlet_p3_beta1e3.txt};
    \addlegendentry{$p=3$};


    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x index = 0, y index = 2] {\dataDir/plate_weak_dirichlet_p4_beta1e3.txt};
    \addlegendentry{$p=4$};

    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
    table[ x index = 0, y index = 2] {\dataDir/plate_weak_dirichlet_p5_beta1e3.txt};
    \addlegendentry{$p=5$};

    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
    table[ x index = 0, y index = 2] {\dataDir/plate_weak_dirichlet_p6_beta1e3.txt};
    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
\logLogSlopeTriangle{0.19}{0.08}{0.25}{2}{black};
\logLogSlopeTriangle{0.19}{0.08}{0.085}{1}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.095}{5}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.095}{6}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.095}{7}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_weak_penalty_h1_beta1e6.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^1$ semi-norm,
%xlabel= Mesh size $h$,
xlabel= mesh size $h$,
legend style={font=\tiny},
legend pos= north west
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x index = 0, y index = 2] {\dataDir/plate_weak_dirichlet_p2_beta1e6.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x index = 0, y index = 2] {\dataDir/plate_weak_dirichlet_p3_beta1e6.txt};
    \addlegendentry{$p=3$};


    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x index = 0, y index = 2] {\dataDir/plate_weak_dirichlet_p4_beta1e6.txt};
    \addlegendentry{$p=4$};

    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
    table[ x index = 0, y index = 2] {\dataDir/plate_weak_dirichlet_p5_beta1e6.txt};
    \addlegendentry{$p=5$};

    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
    table[ x index = 0, y index = 2] {\dataDir/plate_weak_dirichlet_p6_beta1e6.txt};
    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
\logLogSlopeTriangle{0.2}{0.1}{0.075}{1}{black};
\logLogSlopeTriangle{0.19}{0.08}{0.54}{2}{black};
\logLogSlopeTriangle{0.19}{0.08}{0.23}{3}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.095}{5}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.095}{6}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.095}{7}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_weak_penalty_h2_beta1e12.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^2$ semi-norm,
%xlabel= Mesh size $h$,
xlabel= mesh size $h$,
legend style={font=\tiny},
legend pos= south east
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p2_beta1e12.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p3_beta1e12.txt};
    \addlegendentry{$p=3$};


    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p4_beta1e12.txt};
    \addlegendentry{$p=4$};

    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
    \addlegendentry{$p=5$};

    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
\logLogSlopeTriangle{0.19}{0.08}{0.78}{1}{black};
\logLogSlopeTriangle{0.19}{0.08}{0.59}{2}{black};
\logLogSlopeTriangle{0.19}{0.08}{0.41}{3}{black};
\logLogSlopeTriangle{0.19}{0.08}{0.245}{4}{black};
\logLogSlopeTriangle{0.19}{0.08}{0.0825}{5}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_weak_penalty_h2_beta1e3.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^2$ semi-norm,
%xlabel= Mesh size $h$,
xlabel= mesh size $h$,
legend style={font=\tiny},
legend pos= south east
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p2_beta1e3.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p3_beta1e3.txt};
    \addlegendentry{$p=3$};


    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p4_beta1e3.txt};
    \addlegendentry{$p=4$};

    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e3.txt};
    \addlegendentry{$p=5$};

    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e3.txt};
    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
\logLogSlopeTriangle{0.19}{0.08}{0.605}{1}{black};
\logLogSlopeTriangle{0.19}{0.08}{0.1605}{2}{black};
\logLogSlopeTriangle{0.21}{0.1}{0.07}{1}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.095}{1}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.095}{5}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.095}{6}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.095}{7}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_weak_penalty_h2_beta1e6.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^2$ semi-norm,
%xlabel= Mesh size $h$,
xlabel= mesh size $h$,
legend style={font=\tiny},
legend pos= south east
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p2_beta1e6.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p3_beta1e6.txt};
    \addlegendentry{$p=3$};


    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p4_beta1e6.txt};
    \addlegendentry{$p=4$};

    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p5_beta1e6.txt};
    \addlegendentry{$p=5$};

    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
    table[ x index = 0, y index = 3] {\dataDir/plate_weak_dirichlet_p6_beta1e6.txt};
    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
\logLogSlopeTriangle{0.19}{0.08}{0.725}{1}{black};
\logLogSlopeTriangle{0.19}{0.08}{0.47}{2}{black};
\logLogSlopeTriangle{0.19}{0.08}{0.215}{3}{black};
\logLogSlopeTriangle{0.195}{0.1}{0.075}{1}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.095}{5}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.095}{6}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.095}{7}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_weak_penalty_l2_beta1e12.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $L^2$ norm,
%xlabel= Mesh size $h$,
xlabel= mesh size $h$,
legend style={font=\tiny},
legend pos= south east
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x index = 0, y index = 1] {\dataDir/plate_weak_dirichlet_p2_beta1e12.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x index = 0, y index = 1] {\dataDir/plate_weak_dirichlet_p3_beta1e12.txt};
    \addlegendentry{$p=3$};

    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x index = 0, y index = 1] {\dataDir/plate_weak_dirichlet_p4_beta1e12.txt};
    \addlegendentry{$p=4$};

    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
    table[ x index = 0, y index = 1] {\dataDir/plate_weak_dirichlet_p5_beta1e12.txt};
    \addlegendentry{$p=5$};

    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
    table[ x index = 0, y index = 1] {\dataDir/plate_weak_dirichlet_p6_beta1e12.txt};
    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
\logLogSlopeTriangle{0.155}{0.08}{0.655}{2}{black};
\logLogSlopeTriangle{0.155}{0.08}{0.32}{4}{black};
%\logLogSlopeTriangle{0.635}{0.08}{0.325}{5}{black};
%\logLogSlopeTriangle{0.635}{0.08}{0.325}{6}{black};
\logLogSlopeTriangle{0.55}{0.08}{0.2}{7}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_weak_penalty_l2_beta1e3.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $L^2$ norm,
%xlabel= Mesh size $h$,
xlabel= mesh size $h$,
legend style={font=\tiny},
legend pos= south east
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x index = 0, y index = 1] {\dataDir/plate_weak_dirichlet_p2_beta1e3.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x index = 0, y index = 1] {\dataDir/plate_weak_dirichlet_p3_beta1e3.txt};
    \addlegendentry{$p=3$};

    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x index = 0, y index = 1] {\dataDir/plate_weak_dirichlet_p4_beta1e3.txt};
    \addlegendentry{$p=4$};

    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
    table[ x index = 0, y index = 1] {\dataDir/plate_weak_dirichlet_p5_beta1e3.txt};
    \addlegendentry{$p=5$};

    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
    table[ x index = 0, y index = 1] {\dataDir/plate_weak_dirichlet_p6_beta1e3.txt};
    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
\logLogSlopeTriangle{0.19}{0.08}{0.08}{1}{black};
\logLogSlopeTriangle{0.19}{0.08}{0.2575}{2}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.095}{5}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.095}{6}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.095}{7}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_weak_penalty_l2_beta1e6.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $L^2$ norm,
%xlabel= Mesh size $h$,
xlabel= mesh size $h$,
legend style={font=\tiny},
legend pos= north west
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x index = 0, y index = 1] {\dataDir/plate_weak_dirichlet_p2_beta1e6.txt};
    \addlegendentry{$p=2$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x index = 0, y index = 1] {\dataDir/plate_weak_dirichlet_p3_beta1e6.txt};
    \addlegendentry{$p=3$};

    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x index = 0, y index = 1] {\dataDir/plate_weak_dirichlet_p4_beta1e6.txt};
    \addlegendentry{$p=4$};

    \addplot[color=c4, solid, mark=diamond, mark options={solid}] 
    table[ x index = 0, y index = 1] {\dataDir/plate_weak_dirichlet_p5_beta1e6.txt};
    \addlegendentry{$p=5$};

    \addplot[color=c5, solid, mark=pentagon, mark options={solid}] 
    table[ x index = 0, y index = 1] {\dataDir/plate_weak_dirichlet_p6_beta1e6.txt};
    \addlegendentry{$p=6$};

%    \addplot[color=c6, solid, mark=*, mark options={solid}] table[ x index = 3, y index = 2] {\dataDir/trimming_by_hand_debug_p4_GR.txt};
%    \addlegendentry{estimator, $p_b=5$};

{
\logLogSlopeTriangle{0.155}{0.08}{0.535}{2}{black};
\logLogSlopeTriangle{0.425}{0.08}{0.225}{4}{black};
\logLogSlopeTriangle{0.21}{0.1}{0.085}{1}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.095}{6}{black};
%\logLogSlopeTriangle{0.19}{0.08}{0.095}{7}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_weak_rotations_h2_smooth_adaptive.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^2$ semi-norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x index = 0, y index = 2] {\dataDir/shell_weak_dirichlet_p3_THB_MS_bubbles.txt};
    \addlegendentry{error $p=3$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x index = 0, y index = 2] {\dataDir/shell_weak_dirichlet_p4_THB_MS_bubbles.txt};
    \addlegendentry{error $p=4$};


    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x index = 0, y index = 2] {\dataDir/shell_weak_dirichlet_p5_THB_MS_bubbles.txt};
    \addlegendentry{error $p=5$};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x index = 0, y expr=\thisrowno{3}*3.5] {\dataDir/shell_weak_dirichlet_p3_THB_MS_bubbles.txt};
    \addlegendentry{estimator $p_b=4$};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x index = 0, y expr=\thisrowno{3}*3.5] {\dataDir/shell_weak_dirichlet_p4_THB_MS_bubbles.txt};
    \addlegendentry{estimator $p_b=5$};

    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x index = 0, y expr=\thisrowno{3}*3.5] {\dataDir/shell_weak_dirichlet_p5_THB_MS_bubbles.txt};
    \addlegendentry{estimator $p_b=6$};

{
\logLogSlopeReverseTriangle{0.82}{0.08}{0.525}{2}{black};
\logLogSlopeReverseTriangle{0.82}{0.08}{0.27}{3}{black};
\logLogSlopeReverseTriangle{0.82}{0.08}{0.057}{4}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/convergence_weak_rotations_h2_smooth_uniform.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
ymode=log,
%ymin=1e-07,
%ymax=0.1,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Error in $H^2$ semi-norm,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= south west
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x index = 0, y index = 2] {\dataDir/shell_weak_dirichlet_p3_THB_GR_bubbles.txt};
    \addlegendentry{error $p=3$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x index = 0, y index = 2] {\dataDir/shell_weak_dirichlet_p4_THB_GR_bubbles.txt};
    \addlegendentry{error $p=4$};


    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x index = 0, y index = 2] {\dataDir/shell_weak_dirichlet_p5_THB_GR_bubbles.txt};
    \addlegendentry{error $p=5$};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x index = 0, y expr=\thisrowno{3}*3.5] {\dataDir/shell_weak_dirichlet_p3_THB_GR_bubbles.txt};
    \addlegendentry{estimator $p_b=4$};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x index = 0, y expr=\thisrowno{3}*3.5] {\dataDir/shell_weak_dirichlet_p4_THB_GR_bubbles.txt};
    \addlegendentry{estimator $p_b=5$};

    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x index = 0, y expr=\thisrowno{3}*3.5] {\dataDir/shell_weak_dirichlet_p5_THB_GR_bubbles.txt};
    \addlegendentry{estimator $p_b=6$};

{
\logLogSlopeReverseTriangle{0.82}{0.08}{0.53}{2}{black};
\logLogSlopeReverseTriangle{0.82}{0.08}{0.285}{3}{black};
\logLogSlopeReverseTriangle{0.82}{0.08}{0.0675}{4}{black};
}
\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/pcg_condest_laplace_curved_nonconforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
%ymode=log,
%ymin=8e-1,
%ymax=2,
yminorticks=true,
axis background/.style={fill=white},
ylabel= Condition number,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= north west,
%skip coords between index={7}{8}
]

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_FD_1e4_condest_p2.txt};
    \addlegendentry{$p=2$, approx. Schur};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_FD_1e4_condest_p3.txt};
    \addlegendentry{$p=3$, approx. Schur};

    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_FD_1e4_condest_p4.txt};
    \addlegendentry{$p=4$, approx. Schur};

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_FD_exact_schur_1e4_condest_p2.txt};
    \addlegendentry{$p=2$, exact Schur};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_FD_exact_schur_1e4_condest_p3.txt};
    \addlegendentry{$p=3$, exact Schur};

    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_FD_exact_schur_1e4_condest_p4.txt};
    \addlegendentry{$p=4$, exact Schur};



\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/pcg_iter_bilaplace_curved_nonconforming_FD.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
%ymode=log,
ymin=0,
ymax=20,
yminorticks=true,
axis background/.style={fill=white},
ylabel= FGMRES iterations,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= north west,
%skip coords between index={7}{8}
]

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 5] {\dataDir/bilaplace_penalty_non_matching_proj_FD_1e4_condest_p2.txt};
    \addlegendentry{$p=2, tol=10^{-4}$};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 5] {\dataDir/bilaplace_penalty_non_matching_proj_FD_1e4_condest_p3.txt};
    \addlegendentry{$p=3, tol=10^{-4}$};

    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 5] {\dataDir/bilaplace_penalty_non_matching_proj_FD_1e4_condest_p4.txt};
    \addlegendentry{$p=4, tol=10^{-4}$};

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 5] {\dataDir/bilaplace_penalty_non_matching_proj_FD_1e5_condest_p2.txt};
    \addlegendentry{$p=2, tol=10^{-5}$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 5] {\dataDir/bilaplace_penalty_non_matching_proj_FD_1e5_condest_p3.txt};
    \addlegendentry{$p=3, tol=10^{-5}$};


    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 5] {\dataDir/bilaplace_penalty_non_matching_proj_FD_1e5_condest_p4.txt};
    \addlegendentry{$p=4, tol=10^{-5}$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 5] {\dataDir/bilaplace_penalty_non_matching_proj_FD_1e6_condest_p2.txt};
    \addlegendentry{$p=2, tol=10^{-6}$};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 5] {\dataDir/bilaplace_penalty_non_matching_proj_FD_1e6_condest_p3.txt};
    \addlegendentry{$p=3, tol=10^{-6}$};

    \addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 5] {\dataDir/bilaplace_penalty_non_matching_proj_FD_1e6_condest_p4.txt};
    \addlegendentry{$p=4, tol=10^{-6}$};

\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/pcg_iter_bilaplace_curved_nonconforming_FD_exact_schur.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.4\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
%ymode=log,
ymin=0,
ymax=10,
yminorticks=true,
axis background/.style={fill=white},
ylabel= FGMRES iterations,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= north west,
%skip coords between index={7}{8}
]


	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 5] {\dataDir/bilaplace_penalty_non_matching_proj_FD_exact_Schur_1e5_condest_p2.txt};
    \addlegendentry{$p=2$, exact Schur};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 5] {\dataDir/bilaplace_penalty_non_matching_proj_FD_exact_Schur_1e5_condest_p3.txt};
    \addlegendentry{$p=3$, exact Schur};

    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 5] {\dataDir/bilaplace_penalty_non_matching_proj_FD_exact_Schur_1e5_condest_p4.txt};
    \addlegendentry{$p=4$, exact Schur};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 5] {\dataDir/bilaplace_penalty_non_matching_proj_FD_1e5_condest_p2.txt};
    \addlegendentry{$p=2$, approx. Schur};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 5] {\dataDir/bilaplace_penalty_non_matching_proj_FD_1e5_condest_p3.txt};
    \addlegendentry{$p=3$, approx. Schur};

    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 5] {\dataDir/bilaplace_penalty_non_matching_proj_FD_1e5_condest_p4.txt};
    \addlegendentry{$p=4$, approx. Schur};

\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/pcg_iter_bilaplace_curved_nonconforming_ILU.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
%ymode=log,
ymin=0,
ymax=20,
yminorticks=true,
axis background/.style={fill=white},
ylabel= FGMRES iterations,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= north west,
%skip coords between index={7}{8}
]


	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 5] {\dataDir/bilaplace_penalty_non_matching_proj_ILU_1e4_condest_p2.txt};
    \addlegendentry{$p=2, tol=10^{-4}$};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 5] {\dataDir/bilaplace_penalty_non_matching_proj_ILU_1e4_condest_p3.txt};
    \addlegendentry{$p=3, tol=10^{-4}$};

    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 5] {\dataDir/bilaplace_penalty_non_matching_proj_ILU_1e4_condest_p4.txt};
    \addlegendentry{$p=4, tol=10^{-4}$};

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 5] {\dataDir/bilaplace_penalty_non_matching_proj_ILU_1e5_condest_p2.txt};
    \addlegendentry{$p=2, tol=10^{-5}$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 5] {\dataDir/bilaplace_penalty_non_matching_proj_ILU_1e5_condest_p3.txt};
    \addlegendentry{$p=3, tol=10^{-5}$};

    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 5] {\dataDir/bilaplace_penalty_non_matching_proj_ILU_1e5_condest_p4.txt};
    \addlegendentry{$p=4, tol=10^{-5}$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 5] {\dataDir/bilaplace_penalty_non_matching_proj_ILU_1e6_condest_p2.txt};
    \addlegendentry{$p=2, tol=10^{-6}$};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 5] {\dataDir/bilaplace_penalty_non_matching_proj_ILU_1e6_condest_p3.txt};
    \addlegendentry{$p=3, tol=10^{-6}$};

    \addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 5] {\dataDir/bilaplace_penalty_non_matching_proj_ILU_1e6_condest_p4.txt};
    \addlegendentry{$p=4, tol=10^{-6}$};

\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/pcg_iter_bilaplace_curved_nonconforming_ILU_exact_schur.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
%ymode=log,
ymin=0,
ymax=20,
yminorticks=true,
axis background/.style={fill=white},
ylabel= FGMRES iterations,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= north west,
%skip coords between index={7}{8}
]

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 5] {\dataDir/bilaplace_penalty_non_matching_proj_ILU_exact_Schur_1e5_condest_p2.txt};
    \addlegendentry{$p=2$, exact Schur};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 5] {\dataDir/bilaplace_penalty_non_matching_proj_ILU_exact_Schur_1e5_condest_p3.txt};
    \addlegendentry{$p=3$, exact Schur};

    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 5] {\dataDir/bilaplace_penalty_non_matching_proj_ILU_exact_Schur_1e5_condest_p4.txt};
    \addlegendentry{$p=4$, exact Schur};

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{4}^0.5, y index = 5] {\dataDir/bilaplace_penalty_non_matching_proj_ILU_1e5_condest_p2.txt};
    \addlegendentry{$p=2$, approx. Schur};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 5] {\dataDir/bilaplace_penalty_non_matching_proj_ILU_1e5_condest_p3.txt};
    \addlegendentry{$p=3$, approx. Schur};

    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{4}^0.5, y index = 5] {\dataDir/bilaplace_penalty_non_matching_proj_ILU_1e5_condest_p4.txt};
    \addlegendentry{$p=4$, approx. Schur};


\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/pcg_iter_laplace_curved_nonconforming.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
%ymode=log,
%ymin=8e-1,
%ymax=2,
yminorticks=true,
axis background/.style={fill=white},
ylabel= PCG iterations,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= north west,
%skip coords between index={7}{8}
]

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_ILU_1e2_condest_p2.txt};
    \addlegendentry{$p=2, tol=10^{-2}$};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_ILU_1e2_condest_p3.txt};
    \addlegendentry{$p=3, tol=10^{-2}$};

    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_ILU_1e2_condest_p4.txt};
    \addlegendentry{$p=4, tol=10^{-2}$};

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_ILU_1e4_condest_p2.txt};
    \addlegendentry{$p=2, tol=10^{-4}$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_ILU_1e4_condest_p3.txt};
    \addlegendentry{$p=3, tol=10^{-4}$};

    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_ILU_1e4_condest_p4.txt};
    \addlegendentry{$p=4, tol=10^{-4}$};



\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/pcg_iter_laplace_curved_nonconforming_FD.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
%ymode=log,
%ymin=8e-1,
ymax=20,
yminorticks=true,
axis background/.style={fill=white},
ylabel= PCG iterations,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= north west,
%skip coords between index={7}{8}
]

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_FD_1e2_condest_p2.txt};
    \addlegendentry{$p=2, tol=10^{-2}$};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_FD_1e2_condest_p3.txt};
    \addlegendentry{$p=3, tol=10^{-2}$};

    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_FD_1e2_condest_p4.txt};
    \addlegendentry{$p=4, tol=10^{-2}$};

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_FD_1e4_condest_p2.txt};
    \addlegendentry{$p=2, tol=10^{-4}$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_FD_1e4_condest_p3.txt};
    \addlegendentry{$p=3, tol=10^{-4}$};

    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_FD_1e4_condest_p4.txt};
    \addlegendentry{$p=4, tol=10^{-4}$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_FD_1e6_condest_p2.txt};
    \addlegendentry{$p=2, tol=10^{-6}$};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_FD_1e6_condest_p3.txt};
    \addlegendentry{$p=3, tol=10^{-6}$};

    \addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_FD_1e6_condest_p4.txt};
    \addlegendentry{$p=4, tol=10^{-6}$};

\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/pcg_iter_laplace_curved_nonconforming_FD_exact_schur.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
%ymode=log,
%ymin=8e-1,
ymax=10,
yminorticks=true,
axis background/.style={fill=white},
ylabel= FGMRES iterations,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= north west,
%skip coords between index={7}{8}
]


	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_FD_1e4_condest_p2.txt};
    \addlegendentry{$p=2$, approx. Schur};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_FD_1e4_condest_p3.txt};
    \addlegendentry{$p=3$, approx. Schur};

    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_FD_1e4_condest_p4.txt};
    \addlegendentry{$p=4$, approx. Schur};

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_FD_exact_schur_1e4_condest_p2.txt};
    \addlegendentry{$p=2$, exact Schur};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_FD_exact_schur_1e4_condest_p3.txt};
    \addlegendentry{$p=3$, exact Schur};

    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_FD_exact_schur_1e4_condest_p4.txt};
    \addlegendentry{$p=4$, exact Schur};


\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/pcg_iter_laplace_curved_nonconforming_ILU.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
%ymode=log,
%ymin=8e-1,
%ymax=2,
yminorticks=true,
axis background/.style={fill=white},
ylabel= PCG iterations,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= north west,
%skip coords between index={7}{8}
]

	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_ILU_1e2_condest_p2.txt};
    \addlegendentry{$p=2, tol=10^{-2}$};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_ILU_1e2_condest_p3.txt};
    \addlegendentry{$p=3, tol=10^{-2}$};

    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_ILU_1e2_condest_p4.txt};
    \addlegendentry{$p=4, tol=10^{-2}$};

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_ILU_1e4_condest_p2.txt};
    \addlegendentry{$p=2, tol=10^{-4}$};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_ILU_1e4_condest_p3.txt};
    \addlegendentry{$p=3, tol=10^{-4}$};

    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_ILU_1e4_condest_p4.txt};
    \addlegendentry{$p=4, tol=10^{-4}$};

	\addplot [color=c1, dotted,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_ILU_1e6_condest_p2.txt};
    \addlegendentry{$p=2, tol=10^{-6}$};
	
	\addplot[color=c2, dotted, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_ILU_1e6_condest_p3.txt};
    \addlegendentry{$p=3, tol=10^{-6}$};

    \addplot[color=c3, dotted, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_ILU_1e6_condest_p4.txt};
    \addlegendentry{$p=4, tol=10^{-6}$};

\end{axis}
\end{tikzpicture}%



==> pictures/numericalExamples/graphs/pcg_iter_laplace_curved_nonconforming_ILU_exact_schur.tex <==

%
%    \logLogSlopeTriangleOne{0.85}{-0.1}{0.70}{2}{black, semithick};  
%
%    \logLogSlopeTriangleTwo{0.85}{-0.1}{0.42}{3}{black, semithick};
%
%    \logLogSlopeTriangleThree{0.65}{-0.1}{0.30}{4}{black, semithick};  

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{compat=newest}

\usetikzlibrary{calc}
%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C)-- node[pos=0.5,anchor=west] {#4}
                    cycle;
    }
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

\newcommand{\logLogSlopeReverseTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1+#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {\scriptsize 1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=east] {\scriptsize #4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.

%%%%%%% version with mesh size

\begin{tikzpicture}

\begin{axis}[%
width=0.8\textwidth,
height=6.5cm,
at={(0in,0in)},
scale only axis,
xmode=log,
%xmin=1e1,
%xmax=1e0,
xminorticks=true,
%ymode=log,
%ymin=8e-1,
ymax=10,
yminorticks=true,
axis background/.style={fill=white},
ylabel= FGMRES iterations,
%xlabel= Mesh size $h$,
xlabel= $\sqrt{\text{dofs}}$,
legend style={font=\tiny},
legend pos= north west,
%skip coords between index={7}{8}
]


	\addplot [color=c1, dashed,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_ILU_1e4_condest_p2.txt};
    \addlegendentry{$p=2$, approx. Schur};
	
	\addplot[color=c2, dashed, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_ILU_1e4_condest_p3.txt};
    \addlegendentry{$p=3$, approx. Schur};

    \addplot[color=c3, dashed, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_ILU_1e4_condest_p4.txt};
    \addlegendentry{$p=4$, approx. Schur};

	\addplot [color=c1, solid,mark=o,mark options={solid}]
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_ILU_exact_schur_1e4_condest_p2.txt};
    \addlegendentry{$p=2$, exact Schur};
	
	\addplot[color=c2, solid, mark=square, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_ILU_exact_schur_1e4_condest_p3.txt};
    \addlegendentry{$p=3$, exact Schur};

    \addplot[color=c3, solid, mark=triangle, mark options={solid}] 
    table[ x expr=\thisrowno{3}^0.5, y index = 4] {\dataDir/laplace_penalty_non_matching_proj_ILU_exact_schur_1e4_condest_p4.txt};
    \addlegendentry{$p=4$, exact Schur};

\end{axis}
\end{tikzpicture}%



==> sections/BubbleEstimator.tex <==
\newcommand{\picsDir}{pictures/numericalExamples/pics}
\newtheorem{remark}{Remark}

\section{A posteriori error estimator for Kirchhoff plates and Kirchhoff-Love shells} \label{sec:bubbles}

In the following Section we introduce a variant of the error estimator analyzed in \citep{Bank1993} and we extend its isogeometric version, proposed in \citep{Juettler2010}, to fourth-order PDEs of mechanical relevance, such as Kirchhoff plates and Kirchhoff-Love shells. We choose these models since, due to the Kirchhoff hypotheses, we avoid a priori the negative effects related to shear locking. Then, later in the Section, we show a possible implementation of the proposed indicator in the context of hierarchical B-splines.

\subsection{The bubble error estimator}
%The main idea of this family of \textit{a posteriori} estimates is based on the original paper of \citep{Bank1993} 
This family of \textit{a posteriori} estimators was introduced in \citep{Bank1993} in the context of the p-version of the Finite Element Method and has been successfully applied to T-splines in \citep{Juettler2010} for second-order boundary value problems. To introduce the concept in the context of hierarchical IGA, let us define the finite dimensional solution space $V^p_h$ as the span of hierarchical B-splines basis functions of order $p$, where we restrict our analysis to the case $p > 2$ (see Remark~\ref{rem:2} for the case $p =2$). Then, let us recall the discrete solution $u_h \in V^p_h$, where without loss of generality we make no distinction between the plate or the shell problem. We now assume there exists a larger space $V^p_h \subset \widetilde{V}^p_h \subset V$ such that the following decomposition holds:
\begin{align*}
\widetilde{V}^p_h = V^p_h \oplus W^{p+1}_h \, ,
\end{align*} 
where $W^{p+1}_h$ is the space in which we seek a good estimation of the error $e_h \approx e = \left\lVert u - u_h \right\rVert$, in a suitable norm $\left\lVert \cdot \right\rVert$. In particular, recalling some definitions provided in Section \ref{sec:IGA}, let us characterize $W^{p+1}_h$ as follows:
\begin{align*}
W^{p+1}_{h} = \bigcup_{l=0}^N W^{p+1}_{h,l} \, ,
\end{align*}
where 
%\begin{align*}
%W^{p+1}_{h,l} = \text{span }\lbrace b \circ \mathbf{S}^{-1} \vert \, b \in \mathcal{B}^l_{a,p+1} \cap C^1 ( \overbar{\hat{\Omega}^l} ),  \text{ supp}(b) = \overbar{\mathcal{Q}^l} \subset  \overbar{\hat{\Omega}^l} \rbrace.
%\end{align*}
\begin{align*}
W^{p+1}_{h,l} = \text{span }\lbrace b \circ \mathbf{S}^{-1} \vert \, b \in \mathcal{B}^l_{a,p+1} \cap C^1 ( \overbar{\hat{\Omega}^l} )  \text{ and } \exists \, \epsilon \subseteq \hat{\Omega}^l : \text{ supp}(b) = \overbar{\epsilon} \rbrace.
\end{align*}
%\begin{align*}
%W^{p+1}_h = \text{span }\lbrace b_h \circ \mathbf{S}^{-1} \vert \, b_h \in \mathcal{B}^l_{a,p+1} \cap C^1 ( \overbar{\hat{\Omega}^l} ),  \text{ supp}(b_h) = \overbar{\mathcal{Q}^l_i} \subset  \overbar{\hat{\Omega}^l} \rbrace.
%\end{align*}
In words, $W^{p+1}_{h,l}$ is the space spanned by active B-splines (or better in this case, Bernstein polynomials) of level $l$ and degree $p+1$ such that their support is compact and overlaps exactly with one active element $\epsilon$ of level $l$, e.g. see~\Cref{fig:bubble_basis} where one level is depicted.
We are now ready to define the a posteriori error estimate as: find $e_h  \in \: W^{p+1}_h$ such that
% \begin{align}\label{eq:bubbleSystem}
% %&\text{Find} \: e_h  \in \: W^{p+1}_h \text{ such that} \nonumber\\
% &a(e_h,b_h) = F(b_h) - a(u_h,b_h)  \qquad \forall b_h \in W^{p+1}_h 
% \end{align}
%where $b_h$ is referred to in the following as \textit{bubble functions}. We remark that we require these functions to be at least $C^1$ on their support such that the corresponding bilinear form $a$ is well-defined. Notice that due to the compact support property of $b_h$, the linear system corresponding to the discrete error weak form \eqref{eq:bubbleSystem} is block diagonal and in general easy to solve. Once we have found the unknown coefficients $e_h$, we define the element-wise error estimator $\eta_{\epsilon}$ as follows:
%\begin{align*}
%\eta_{\epsilon} = C_a \left\lVert e_h \right\rVert_{E(\epsilon)}  \quad \forall \epsilon \in \mathcal{E} \, ,
%\end{align*}
%\begin{subequations}\label{eq:bubbleProblem}
 \begin{equation}\label{eq:bubbleSystem}
 %&\text{Find} \: e_h  \in \: W^{p+1}_h \text{ such that} \nonumber\\
 a(e_h,b_h) = F(b_h) - a(u_h,b_h)  \qquad \forall b_h \in W^{p+1}_h  \, ,
 \end{equation}  
where $b_h$ is referred to in the following as \textit{bubble functions}. We remark that we require these functions to be at least $C^1$ on their support such that the corresponding bilinear form $a$ is well-defined. Notice that due to the compact support of $b_h$, the linear system corresponding to the discrete error weak form \eqref{eq:bubbleSystem} is block diagonal and in general easy to solve. 
Moreover, we highlight that the evaluation of the bilinear form $a$ appearing in~\eqref{eq:bubbleSystem} follows the same steps as the original plate/shell problem, where different test functions $b_h$ are used. Hence, setting up the bubble problem requires only minor changes into an existing isogeometric code.    

Once we have found the unknown coefficients $e_h$, we define the element-wise error estimator $\eta_{\epsilon}$ as follows:
\begin{equation}\label{eq:bubbleSystem_bis}
\eta_{\epsilon} = C_a \left\lVert e_h \right\rVert_{E(\epsilon)}  \quad \forall \epsilon \in Q \, ,
\end{equation}  
%\end{subequations}
where we recall that $\epsilon$ is an isogeometric element of the hierarchical mesh $Q$ and $\left\lVert \cdot \right\rVert_{E(\epsilon)}$ denotes the energy norm restricted to element $\epsilon$. Additionally, we introduce $C_a$ as an empirical constant which, considering all our numerical experiments, we claim is independent from the chosen degree and from the problem at hand. In the following, we set $C_a = 3$ once and for all in order to shift the estimator above the true error.

At this point, it is worth highlighting that the proposed error estimator is computationally inexpensive, easy to implement and is embarrassingly parallelizable due to the choice of the disjoint bubble space $W^{p+1}_h$. A possible algorithm to estimate the error is summarized in Algorithm~\ref{alg:estimate}, where we design the code to solve the additional problem \eqref{eq:bubbleSystem} level-wise over the hierarchical mesh $Q$.

\begin{algorithm}[H] 
\begin{algorithmic}[1]
	\Procedure{Estimate error }{numerical solution $u_h$, hierarchical mesh $Q$} %, $\mathcal{HB}$
	\State Initialize vector $\eta$
	\For{\textbf{each} level $l$ of $Q$}
		\State Build bubble space $W^{p+1}_{h,l}$
		%\For{\textbf{each} active elements $\epsilon$ of level $l$}
		%\For{\textbf{each} $\epsilon \in \mathcal{E}^l$}
		%	\State Compute the bubble shapes corresponding to element $\epsilon$
		%\EndFor
		\State Given $u_h$, get $u_h^l$ of level $l$
		\State Given $u_h^l$, set up and solve the additional system \eqref{eq:bubbleSystem}
		\For{\textbf{each} $\epsilon \in Q^l$}
			\State Compute the element-wise indicator $\eta_{\epsilon}$ \eqref{eq:bubbleSystem_bis}
			\State Store $\eta_{\epsilon}$ in $\eta$
		\EndFor
	\EndFor	
	\State Return $\eta$
	\EndProcedure
\end{algorithmic} 
\caption{Bubble error estimator algorithm}\label{alg:estimate}
\end{algorithm}

\begin{remark}[Inhomogeneous boundary conditions]
On one hand, we highlight that whenever inhomogeneous boundary conditions of Neumann-type are applied to the problem at hand, problem \eqref{eq:bubbleSystem} must also contain the corresponding additional terms in the right-hand-side. In these cases, we augment the bubble space $W^{p+1}_h$ with suitable boundary bubbles to properly capture the error on the imposition of natural boundary conditions. An example is depicted in~\Cref{fig:bubble_basis} for bubbles of degree $p=4,5$. On the other hand, we make the assumption that the error on the imposition of inhomogeneous Dirichlet-type boundary conditions is negligible and therefore no additional shape functions are needed for these cases.
\end{remark}

\begin{figure}[!h]
%	\centering
%\fbox{
	\begin{subfigure}[t]{0.475\textwidth}
	\centering
		%\input{\picsDir/bubble_basis_p4.tex}
	\includegraphics[scale=1.0]{\picsDir/bubble_basis_p4.pdf}
	\caption{Bubble basis $p=4$.}
	\label{fig:bubble_basis_p4}
	\end{subfigure}
%	}
	%\hfill
%	\centering
	\begin{subfigure}[t]{0.475\textwidth}
	\centering
		%\input{\picsDir/bubble_basis_p4_withBCs.tex}
	\includegraphics[scale=1.0]{\picsDir/bubble_basis_p4_withBCs.pdf}	
	\caption{Bubble basis $p=4$ with boundary functions.}
	\label{fig:bubble_basis_p4_withBCs}
	\end{subfigure}		
%\end{figure}
%\begin{figure}[!h]
\par\bigskip
%\fbox{
	\begin{subfigure}[t]{0.475\textwidth}
	\centering
		%\input{\picsDir/bubble_basis_p5.tex}
	\includegraphics[scale=1.0]{\picsDir/bubble_basis_p5.pdf}	
	\caption{Bubble basis $p=5$.}
	\label{fig:bubble_basis_p5}
	\end{subfigure}
%	}
	%\hfill
%	\centering
	\begin{subfigure}[t]{0.475\textwidth}
	\centering
		%\input{\picsDir/bubble_basis_p5_withBCs.tex}
	\includegraphics[scale=1.0]{\picsDir/bubble_basis_p5_withBCs.pdf}		
	\caption{Bubble basis $p=5$ with boundary functions.}
	\label{fig:bubble_basis_p5_withBCs}
	\end{subfigure}	
	\caption{Example of construction of bubble functions $b_h$ as tensor product of univariate functions for the case $p=3,4$, where on the left-side only internal functions are depicted whereas on the right-side also boundary functions are plotted.}
	\label{fig:bubble_basis}
\end{figure}

%\begin{remark}[The case $p=2$]
%We should also highlight that the construction of the bubble space $W^{p+1}_h$ is not straightforward in the case where the underlying B-splines are quadratic. We propose as possible remedies:
%\begin{enumerate}
%\item Construction of an additional sub-grid obtained as dyadic refinement of the original hierarchical mesh and definition of the bubble functions on the corresponding space defined by the new grid.
%
%\item Introduction of suitable edge functions in the bubble space.
%\end{enumerate}
%Notice that, although both approaches could be feasible, they add a non-negligible complexity to the method. In the first case, a new, finer hierarchical grid has to be created at every iteration of the adaptive loop and numerical integration of \eqref{eq:bubbleSystem} has to be performed over it. In the second case, the definition of which edge bubbles have to be considered in the hierarchical case is not unique and considerably worsen the simplicity of the method. Indeed, the corresponding linear system would become more difficult to solve since the element-wise locality of the bubble functions would be lost. Finally, we remark that isogeometric Kirchhoff-Love elements notoriously suffer from membrane locking phenomena, specially for low degree discretization \citep{Kiendl2009}. Moreover, in the spirit of a seamless integration of computer aided design (CAD) and IGA, we highlight that the vast majority of geometrical models is built with splines of degree $p=3$, as a matter of example see \citep{Marussig2018} and references therein.
%In light of these considerations, we will not address further the case $p=2$ in the scope of this work.     
%\end{remark}
\begin{remark}[The case $p=2$] \label{rem:2}
We remark that isogeometric Kirchhoff-Love elements notoriously suffer from membrane locking phenomena, specially for low degree discretization \citep{Kiendl2009}, and it can be considered common practice to use the coarsest (and lowest degree) description of the geometry that is still exact while employing a \textit{k}-refined space for the solution field to mitigate these effects. 
%Moreover, in the spirit of a seamless integration of computer aided design (CAD) and IGA, we highlight that the vast majority of geometrical models is built with splines of degree $p=3$, as a matter of example see \citep{Marussig2018} and references therein.
Nevertheless, for the sake of completeness, we should highlight that the construction of the bubble space $W^{p+1}_h$ is not straightforward in the case where the underlying B-splines are quadratic. 
 \noindent We propose as possible remedies:
\begin{enumerate}
\item Construction of an additional sub-grid obtained as dyadic refinement of the original hierarchical mesh and definition of the bubble functions on the corresponding space defined by the new grid.

\item Introduction of suitable edge functions in the bubble space.
\end{enumerate}
Notice that, although both approaches could be feasible, they add a non-negligible complexity to the method. In the first case, a new, finer hierarchical grid has to be created at every iteration of the adaptive loop and numerical integration of \eqref{eq:bubbleSystem} has to be performed over it. In the second case, the definition of which edge bubbles have to be considered in the hierarchical case is not unique and considerably worsen the simplicity of the method. Indeed, the corresponding linear system would become more difficult to solve since the element-wise locality of the bubble functions would be lost. Therefore, 
in light of these considerations, we will not address further the case $p=2$ in the scope of this work.     
\end{remark}

\begin{remark}[Jumps in the residual]
In the last remark, we notice that, although the residual exhibits jumps across element edges for the discretization of degree $p=3$, in all our computations the estimator behaves still optimally even if the corresponding jump terms are not accounted for in \eqref{eq:bubbleSystem}.  
\end{remark}

\subsection{Marking and refine strategies}

Here, we briefly recall that once an estimate of the error element-wise is available, there exist several strategies proposed in the literature to mark elements for refinement. In all our numerical examples we use the so-called \textit{maximum strategy}, which can be summarized as follows. Let $\gamma \in (0,1)$ be a user-defined threshold, all elements such that
\begin{align*}
\eta_{\epsilon} > \gamma \, \tilde{\eta}_{\varepsilon} \, , \quad \text{where} \quad \tilde{\eta}_{\varepsilon} = \max_{\varepsilon \in Q} \, \eta_{\varepsilon} \, ,
\end{align*}
are marked for refinement. In the following, if not stated otherwise, we will always use $\gamma = 0.5$.
Additionally, since for basis functions of order $p$ their support usually spans up to $p+1$ elements, we try to reduce the number of isolated marked elements. Indeed, in general, isolated refined elements do not improve the solution space $V^p_h$ (they do not add any additional degree of freedom) but only the associated numerical integration is refined. To avoid that, we slightly modify the maximum strategy marking algorithm such that once an element $\epsilon$ of level $l$ is marked for refinement, the algorithm also marks all the neighbors of $\epsilon \in Q^l$, where $Q^l$ is the set of active elements of level $l$.
Finally, we remark that our marking algorithm is also designed to preserve the admissibility (as defined in~\citep{Buffa2016a}) of the hierarchical mesh between consecutive iterations of the adaptive loop. We recall that admissible meshes are guaranteed to have a bounded number of basis functions acting on any element of the mesh, such that interaction between very fine and very coarse functions is avoided. 
If not stated otherwise, we will set the class of admissibility $m$ to be $m = p-1$ in all our numerical examples. 
For the sake of brevity we do not discuss the details here, the reader is referred to \citep{Buffa2016a,Buffa2017,Bracco2018} for a comprehensive review of the concept of admissibility.











==> sections/IGA.tex <==
% !TeX root = ../main.tex
\newcommand\superHB{\scriptscriptstyle\mathcal{HB};\;}
\newcommand\superTHB{\scriptscriptstyle\mathcal{THB};\;}
\newcommand{\Norm}[1]{\left\lVert#1\right\rVert_2}
\newcommand{\delom}{{\;\text{d}\Omega}}
\newcommand{\delg}{{\;\text{d}\Gamma}}
\newcommand{\energyNorm}[1]{\left\lVert#1\right\rVert_{E(\Omega)}}
\newcommand{\snot}{{S}}
\newcommand{\s}{{\snot \left( \T, p \right) }}
\newcommand{\T}{{\mathcal{T}}}
\newcommand{\op}{{\Omega\textsuperscript{\text{phy}}}}
\newcommand{\of}{{\Omega\textsuperscript{\text{fict}}}}


%\section{Methods}
%\label{sec:methods}
%In the following section, all the methods that have been combined in our framework are briefly summarized. For more details, references specific to a particular method are given in the corresponding sub-section.

\section{IsoGeometric Analysis} \label{sec:IGA}

\newcommand{\bg}{}
In this Section, the notation and basic concepts and definitions related to B-splines and NURBS are reviewed, following closely the derivation in~\citep{Dangella2018}. For further details, the reader is referred to~\citep{Piegl1995, Cottrell2009}, and references therein.

A B-spline basis function of degree $p$ is generated starting from a non-decreasing sequence of real values that corresponds to a set of coordinates in the parameter space referred to as knot vector, denoted in the following as $\Xi$.
%follows:
%\begin{equation*}
%\Xi=\left\{ \xi_{1},...,\xi_{m+p+1}\right\} 
%\end{equation*}
%where $m \in \mathbb{N}$ represents the number of basis functions. 
Given a knot vector, a univariate B-spline basis function $b_{i,p}$ can be defined recursively using the Cox-de Boor algorithm~\citep{Piegl1995}.
%where $m$ represents the number of basis functions, or equivalently the number of the associated control points. Given a knot vector, a univariate B-spline basis function $N_{i,p}\left(\xi\right)$ can be defined recursively using the Cox-de Boor algorithm. Starting from $p=0$, this reads:%
%\begin{equation*}%
%b_{i,0}\left(\xi\right)=\begin{cases}
%1 & \mathrm{if} \, \, \xi_{i}\leq\xi<\xi_{i+1}\\
%0 & \mathrm{otherwise.}
%\end{cases}%
%\end{equation*}%
%The basis functions for $p>0$ are computed as:
%\begin{equation*}
%b_{i,p}\left(\xi\right)=\frac{\xi-\xi_{i}}{\xi_{i+p}-\xi_{i}}b_{i,p-1}\left(\xi\right)+\frac{\xi_{i+p+1}-\xi}{\xi_{i+p+1}-\xi_{i+1}}b_{i+1,p-1}\left(\xi\right) \, ,
%\end{equation*}
%where the convention $0/0=0$ is used. It is worth mentioning that the smoothness of the obtained B-spline basis is $C^{p-k}$ at every knot, where $k$ denotes the multiplicity of the considered knot, while it is $C^\infty$ everywhere else.
It is worth mentioning that the smoothness of the obtained B-spline basis is $C^{p-k}$ at every knot, where $k$ denotes the multiplicity of the considered knot, while it is $C^\infty$ everywhere else.
%An important category of knot vectors are the so-called open knot vectors, which are standard in computer-aided design (CAD). Open knot vectors are constructed by increasing the multiplicity of the first and the last knots to $k=p+1$, leading to a basis that is interpolatory at both ends, see for instance \Cref{fig:basis_1d_ex}. 
%\begin{figure}
%		\centering
%		\input{pictures/basis/bspline_basis_1d.tikz}
%		\caption{Example of one-dimensional quadratic B-spline basis functions, generated by the open knot vector $\Xi = \{0,0,0,0.25,0.25,0.5,0.75,1,1,1\}$.}
%		\label{fig:basis_1d_ex}
%\end{figure}

%\begin{figure}[htbp]
%	\begin{center}
%		%\includegraphics[scale=0.35]{./plots/cub_basis_fcn.eps}
%		\caption{Cubic B-Spline basis functions formed from the open knot vector $\Xi =
%			\{0,0,0,0,1/6,1/3,1/2,2/3,5/6,1,1,1,1\}$.}
%		\label{fig:basis_ex}
%	\end{center}
%\end{figure}
%
%B-spline curves can then be constructed as follows:
%\begin{equation*}
%\mathbf{C}\left(\xi\right)=\sum_{i=1}^{m}b_{i,p}\mathbf{P}_{i}
%\end{equation*}
%where the coefficients $\mathbf{P}_{i}\in\mathbb{R}^{d}$ of the linear combination are the so-called control
%points and $d$ denotes the dimension of the physical space. %(see, e.g., Figure \ref{fig:curve_ex}).
%\begin{figure}[htbp]
%	\begin{center}
%		%\includegraphics[scale=0.375]{./plots/curve.eps}
%		\caption{A 2D piecewise cubic B-Spline curve generated from the basis functions of Figure \ref{fig:basis_ex} (solid line), along with its control points (black dots), and control net (dotted line)}
%		\label{fig:curve_ex}
%	\end{center}
%\end{figure}
The definition of multivariate B-splines is achieved in a straight-forward manner using the tensor product of univariate B-splines. Indeed, the multivariate B-splines $\mathcal{B}_{\mathbf{i},\mathbf{p}}$ are obtained as:
\begin{equation*}
\mathcal{B}_{\mathbf{i},\mathbf{p}}=\prod_{r=1}^{d_{r}}b_{i_{r},p_{r}}^{r}
\end{equation*}
with $r=1,...,d_{r}$, where $d_{r}$ is the dimension of the parameter space and $p_{r}$ denotes the polynomial degree in the parametric
direction $r$, respectively. Additionally, the multi-index $\mathbf{i}=\left\{ i_{1},...,i_{d_{r}}\right\} $
denotes the position in the tensor product structure and $\mathbf{p}=\left\{ p_{1},...,p_{r}\right\} $
indicates the vector of polynomial degrees. 

%In the scope of this paper, it is of particular interest the case of $d_{r}=2$, which corresponds to B-spline surfaces. Analogously to B-spline curves, they are defined as a linear combination of multivariate B-spline basis functions and control points as follows:
Lastly, let us define a B-spline parametrization $\mathbf{S}$ as a linear combination of multivariate B-spline basis functions and control points as follows:
\begin{equation*}
\mathbf{S}=\sum_{\mathbf{i}}\mathcal{B}_{\mathbf{i},\mathbf{p}}\mathbf{P}_{\mathbf{i}} \, ,
\end{equation*}
%\begin{equation*}
%\mathbf{S}\left(\bg\xi\right)=\sum_{i_2} \sum_{i_2} B_{\mathbf{i},\mathbf{p}}\left(\bg\xi\right)\mathbf{P}_{\mathbf{i}}
%\end{equation*}
where the coefficients $\mathbf{P}_{\mathbf{i}}\in\mathbb{R}^{d}$ of the linear combination are the control points and $d$ denotes the dimension of the physical space. We remark that all the concepts summarized here can be readily transferred to NURBS, for further details we refer to~\citep{Cottrell2009}.
%Let us define NURBS basis functions in $\mathbb{R}^{d}$ through a projective transformation of their B-spline counterparts in $\mathbb{R}^{d+1}$. One-dimensional
%NURBS basis functions $r_{i,p}\left(\xi\right)$ are given by
%\begin{equation*}
%r_{i,p}\left(\xi\right)=\frac{b_{i,p}\left(\xi\right)w_{i}}{\sum_{j=1}^{m}b_{j,p}\left(\xi\right)w_{j}}
%\end{equation*}
%where $b_{i,p}$ are the univariate B-spline basis functions previously introduce and $w_{i}$ are the
%corresponding weights. Finally, multivariate NURBS basis functions are obtained as
%\begin{equation*}
%R_{\mathbf{i},\mathbf{p}}\left(\bg\xi\right)=\frac{B_{\mathbf{i},\mathbf{p}}\left(\bg\xi\right)w_{\mathbf{i}}}{\sum_{\mathbf{j}}B_{\mathbf{j},\mathbf{p}}\left(\bg\xi\right)w_{\mathbf{j}}}
%\end{equation*}
%and NURBS surfaces are constructed as
%\begin{equation*}
%\mathbf{S}\left(\bg\xi\right)=\sum_{\mathbf{i}}R_{\mathbf{i},\mathbf{p}}\left(\bg\xi\right)\mathbf{P}_{\mathbf{i}} \text{.}
%\end{equation*}
In the rest of the paper, without loss of generality, the degree $ p $ will be considered equal in each parametric direction and will be omitted from the notation.

\subsection{Hierarchical B-splines} \label{subsection:hierchical}

In this Subsection, the concept of hierarchical B-spline basis, denoted by $ \mathcal{HB} $, is introduced. This allows us to build a basis that is locally refinable and therefore to overcome the limitations intrinsic to the tensor-product nature of B-splines and NURBS. 

%\subsubsection{Overlay of Univariate B-Splines}
Let $ V^0 \subset V^1 \subset \cdots \subset V^{N} $ be a sequence of nested spaces of splines defined on a parametric domain $ \hat{\Omega}$, where, to keep the notation simple, we consider the one-dimensional case. Each space $ V^l $, $ l=0 ,\ldots, N $ is spanned by the B-spline basis $ \mathcal{B}^l $ of degree $ p $, associated to level $ l $ and the corresponding knot vector $\Xi^l$. 
%Additionally, let $ \Xi^l = ( \xi^l_0, \ldots, \xi^l_{n^l} ) $ be the knot vector composed of non-decreasing real numbers defining the basis $ \mathcal{B}^l $. The nested nature of the spaces $ V^l  $ implies that also the knot vectors are nested, that is, any knot in $ \Xi^l $ is found in $ \Xi^{l+1} $ with at least the same multiplicity, for $ l=0\ldots N-1 $. This is denoted by $ \Xi^{l} \subset \Xi^{l+1} $. An example of hierarchical B-spline basis is shown in \Cref{fig:hierarchicalFunctions}, where three nested knot vectors and their associated overlays of B-spline functions are depicted. 
%In particular, note that each knot in a level $ l $ is present in every knot vector of level $ l^*>l $.

%
%\begin{figure}
%		\centering
%		\begin{subfigure}[t]{\textwidth}
%			\centering
%			\includegraphics[width=\textwidth]{pictures/basis/multiLevelBasis1D.pdf}
%			\vspace{-0.4cm}
%			\caption{Example of hierarchical B-spline functions. The knots of each level are marked by red crosses. Picture adapted from~\citep{Dangella2018}.}
%			\label{fig:hierarchicalFunctions}
%		\end{subfigure}
%		\vspace*{\floatsep}
%		\begin{subfigure}[t]{\textwidth}
%			\centering
%		    \includegraphics[width=\textwidth]{pictures/basis/multiLevelBasisHBElement.pdf}
%			\vspace{-0.4cm}
%		\end{subfigure}
%			\caption{Example of element mesh with associated $ \mathcal{HB} $-spline basis. The elements are marked by the thick red lines on the horizontal axes. $ \mathcal{B}^l_a $ is composed of the colored and of the dotted functions. $ \mathcal{B}^l_- $ is composed of the  dotted functions. $ \mathcal{B}^l_+ $ is composed of the dashed functions. $ \mathcal{B}^l_= $ is composed of the solid non-gray functions. The solid gray functions are inactive. Picture adapted from~\citep{Dangella2018}.}
%		\label{fig:hierarchicalBasis}
%\end{figure}

%\begin{figure}
%		\centering
%		\input{pictures/basis/multiLevelBasis1D.tikz}
%		%%\includegraphics[width=\textwidth]{pictures/basis/multiLevelBasis1D.pdf}
%		\vspace{-0.4cm}
%		\caption{Example of hierarchical B-Spline functions. The knots of each level are marked by red crosses. Picture adapted from~\citep{Dangella2018}.}
%		\label{fig:hierarchicalFunctions}
%		\vspace*{\floatsep}
%		%\input{pictures/basis/multiLevelBasis1DElements.tikz}
%		\input{pictures/basis/multiLevelBasis1DElements.justHB.tikz}
%	    %\includegraphics[width=\textwidth]{pictures/basis/multiLevelBasisHBElement.pdf}
%		\vspace{-0.4cm}
%		\caption{Example of element mesh with associated $ \mathcal{HB} $-spline basis. The elements are marked by the thick red lines on the horizontal axes. $ \mathcal{B}^l_a $ is composed of the colored and of the dotted functions. $ \mathcal{B}^l_- $ is composed of the  dotted functions. $ \mathcal{B}^l_+ $ is composed of the dashed functions. $ \mathcal{B}^l_= $ is composed of the solid non-gray functions. The solid gray functions are inactive. Picture adapted from~\citep{Dangella2018}.}
%		\label{fig:hierarchicalBasis}
%\end{figure}

% Moreover, let $ \mathcal{E}^l_+ = \bigcup_{l^*=l+1}^N \mathcal{E}^l  $ be the set of finer elements of level $ l^*>l $ and  $ \mathcal{E}^l_- = \bigcup_{l^*=0}^{l-1} \mathcal{E}^l $ be the set of coarser elements of level $ l^*<l $.

Our task now is to identify a set of analysis-suitable functions $ \mathcal{N} \subset \bigcup_{l} \mathcal{B}^l $. To this end, let us define as isogeometric elements $Q$ a partition of $ \hat{\Omega} $. In particular, given $\hat n^l \in \mathbb{N}$, let $ \hat \Xi^l = (\hat\xi^l_0, \ldots, \hat \xi^l_{\hat n^l} ) $ be the knot vector composed of non-decreasing knots of $ \Xi^l $ without repetition, and let:
\begin{align*}
\mathcal{Q}^l = \left\lbrace \mathcal{Q}^l_i \;  | \; \mathcal{Q}^l_i = ( \hat \xi^l_i, \hat \xi^l_{i+1} ) , i=0,\ldots, \hat n^l-1 \right\rbrace 
\end{align*}
be the set of open intervals constituting the non-empty knot spans of $ \Xi^l $. The elements of the multi-level mesh can be any non-overlapping partition $ Q \subset \bigcup_{l} \mathcal{Q}^l $ of $ \hat{\Omega} $, such that $\bigcup_{\epsilon \in Q} \bar \epsilon = \hat{\Omega}$.
%
%\begin{itemize}
%	\item $ \emptyset \notin \mathcal{E}, $
%	\item $ \epsilon \in \mathcal{E} \implies \epsilon \in \mathcal{Q}^l, \; \text{for some } 0\leq l \leq N, $
%	\item $ \bigcup \limits_{\epsilon \in \mathcal{E}} \bar \epsilon = \hat{\Omega}, $
%	\item $ \epsilon_1 \cap \epsilon_2 = \emptyset $,   $ \; \forall\epsilon_1, \epsilon_2 \in \mathcal{E}  $,   $ \; \epsilon_1 \neq \epsilon_2 $.
%\end{itemize}%
%
%Here, $  \bar \epsilon $ denotes the closure of $ \epsilon $. 
%Note that we do not consider as elements all the non-empty spans of all levels, but a subset of them that partitions the domain. 
Moreover, let $ Q^l = Q \cap \mathcal{Q}^l $ be the elements of level $ l $, and let $ \hat{\Omega}^l = \bigcup_{\epsilon \in Q^l} \bar \epsilon $ denote their domain. Furthermore, let $ \hat{\Omega}^l_+ = \bigcup_{l^*=l+1}^N  \hat{\Omega}^{l^*} $ be the refined domain with respect to level $ l $ and, analogously, let $ \hat{\Omega}^l_- = \bigcup_{l^*=0}^{l-1}  \hat{\Omega}^{l^*} $ be the coarser domain. 
%For example, \Cref{fig:hierarchicalBasis} shows a possible choice of elements for the knots depicted in \Cref{fig:hierarchicalFunctions}, where we have%
%%\begin{itemize}
%%	\item $ \Omega^0 = [-1, 0] $, $ \Omega^1 = [0, 0.25] $, $ \Omega^2 = [0.25, 1] $,
%%	\item $ \Omega^0_+ = [0, 1] $, $ \Omega^1_+ = [0.25, 1] $, $ \Omega^2_+ = \emptyset $,
%%	\item $ \Omega^0_- = \emptyset $, $ \Omega^1_- = [-1, 0] $, $ \Omega^2_- = [-1, 0.5] $.
%%\end{itemize}
%\[\begin{array}{lllll}
%\hat{\Omega}^0 = [0, 0.5], && \hat{\Omega}^1 = [0.5, 0.625], && \hat{\Omega}^2 = [0.625, 1],\\
%\hat{\Omega}^0_+ = [0.5, 1], && \hat{\Omega}^1_+ = [0.625, 1], &&  \hat{\Omega}^2_+ = \emptyset, \\
%\hat{\Omega}^0_- = \emptyset, && \hat{\Omega}^1_- = [0, 0.5], &&  \hat{\Omega}^2_- = [0, 0.625].\\
%\end{array}\]%
%
\noindent Given a set of elements $Q$, we still need to define a set of basis functions $ \mathcal{N} \subset \bigcup_{l} \mathcal{B}^l $ suitable for analysis. To this end, we consider the set of functions with support on the elements of level $l$ as the set of \emph{active} functions $ \mathcal{B}^l_a =  \left\lbrace b \; |  b \in \mathcal{B}^l, \, \supp{b} \cap \hat{\Omega}^l \neq \emptyset \right\rbrace \subset\mathcal{B}^l $. Among these, a subset of linearly independent functions has to be chosen. Following~\citep{Hennig2016,Dangella2018}, we partition $ \mathcal{B}^l_a $ into:
%\begin{align*}	
%	\mathcal{B}^l_- &=  \left\lbrace b \; |\;  b \in \mathcal{B}^l_a, \, \supp{b} \cap \hat{\Omega}^l_- \neq \emptyset \right\rbrace && \textit{(overlap with coarser elements),} \\
%	 \mathcal{B}^l_+ &=  \left\lbrace b \; |\;  b \in \mathcal{B}^l_a, \, \supp{b} \cap \hat{\Omega}^l_+ \neq \emptyset \right\rbrace \setminus \mathcal{B}^l_- && \textit{(overlap with finer elements, but not with coarser),} \\
% \mathcal{B}^l_= &=  \left\lbrace b \; |\;  b \in \mathcal{B}^l_a, \, \supp{b}  \subset \hat{\Omega}^l  \right\rbrace  && \textit{(overlap just with elements of level $ l $),}
%\end{align*}
\begin{align*}	
	\mathcal{B}^l_- &=  \left\lbrace b \; |\;  b \in \mathcal{B}^l_a, \, \supp{b} \cap \hat{\Omega}^l_- \neq \emptyset \right\rbrace \, , \\
	 \mathcal{B}^l_+ &=  \left\lbrace b \; |\;  b \in \mathcal{B}^l_a, \, \supp{b} \cap \hat{\Omega}^l_+ \neq \emptyset \right\rbrace \setminus \mathcal{B}^l_- \, , \\
 \mathcal{B}^l_= &=  \left\lbrace b \; |\;  b \in \mathcal{B}^l_a, \, \supp{b}  \subset \hat{\Omega}^l  \right\rbrace  \, .
\end{align*}
%
%
%\begin{itemize}	
%	\item overlapping coarser elements: $ \mathcal{B}^l_- =  \left\lbrace b \; |  b \in \mathcal{B}^l_a, \, supp(b) \cap \Omega^l_- \neq \emptyset \right\rbrace $
%	\item overlapping finer elements, but no coarser element: $ \mathcal{B}^l_+ =  \left\lbrace b \; |  b \in \mathcal{B}^l_a, \, supp(b) \cap \Omega^l_+ \neq \emptyset \right\rbrace \setminus \mathcal{B}^l_-$
%	\item overlapping just elements of level $ l $: $ \mathcal{B}^l_= =  \left\lbrace b \; |  b \in \mathcal{B}^l_a, \, supp(b) \subset \Omega^l  \right\rbrace $.
%\end{itemize}
%Such a classification is analogous to the one provided in.
%We are now ready to introduce the Hierarchical B-Splines Basis ($ \mathcal{HB} $).
%\subsubsection{Hierarchical B-Splines Basis}
Then, the hierarchical B-spline basis $ \mathcal{HB} $~\citep{Vuong2011,Kraft1997} is defined as follows:
  \begin{align}
	\label{eq:hb}
	\mathcal{HB} &= \bigcup\limits_l \; \mathcal{HB}^{l}\, ,  \\
	\mathcal{HB}^{l} &= \left( \mathcal{B}^l_= \cup \mathcal{B}^l_+ \right). \nonumber
\end{align}
Namely, $ \mathcal{HB} $ is the set of B-splines of each level $ l $ whose support intersects only elements of level $ \tilde{l} \geq l $ and at least one element of level $ l $. It was proven in~\citep{Vuong2011} that this set is composed of linearly independent functions and therefore suitable for the analysis.





